Harnessing the Power of LLMs: Evaluating Human-AI Text Co-Creation through the Lens of News Headline Generation

To explore how humans can best leverage LLMs for writing and how interacting with these models affects feelings of ownership and trust in the writing process, we compared common human-AI interaction types (e.g., guiding system, selecting from system outputs, post-editing outputs) in the context of LLM-assisted news headline generation. While LLMs alone can generate satisfactory news headlines, on average, human control is needed to fix undesirable model outputs. Of the interaction methods, guiding and selecting model output added the most benefit with the lowest cost (in time and effort). Further, AI assistance did not harm participants' perception of control compared to freeform editing.

==> Results/Task-diff-thematic/con0.tex <==
Con 0
Positive - Interface design (5)

It was not difficult to create headlines. Having the headline box and article side by side was helpful. An improvement might be having the headline box about the news article so the articles isn't squished on the side and the layout is more natural.

Being able to read and scroll through the article made it easy to put my ideas down and continue reading to make any edits.

The System was easy to use. It was hard to think of names for some of the articles.

The articles were not that long, enough information was present to construct headlines

it an easy system to use
Positive - Article content (4)

Most were short and easy reads with clear points and subjects.

Headlines are easier to write when an article is easier to read has has a good flow of events

Writing headlines is second nature to me. For the articles with a strong lead, I was able to skim the rest of the article and find the important information right away. It was not hard to find the important details and convey them with the headline.

The articles were very to the point and it was not hard to come up with a good headline for the articles.
Negative - Difficulty in coming up with headlines (1)

The System was easy to use. It was hard to think of names for some of the articles.
Negative - Difficulty in using interface (1)
 
The system made it very difficult at first because it was hard to read the articles once I clicked to the page where I was to actually create the headlines. It did get easier when I wrote the headlines on a piece of paper while I was still on the screen where it was easy to read the article.

==> Results/Task-diff-thematic/con1.tex <==
Con 1
Positive - Full generator (2)

It was easier creating the headlines with the system

It was quite easy!
Positive - Headline generation (3)

My "Creation" was simply limited to selecting 1 of 3 choices, so "Creation" was incredibly easy.

For most articles, the system provided useful article titles, and it was easy to select the most effective ones.

I do not think it was difficult to create the headlines for the news articles with the system because the system's creation of headlines tends to have pretty clear patterns like creating ones that are either too general/vague or too wordy/unclear. Through process of elimination, it was usually pretty easy to pick the headline that both conveys the main point of the article and has clear use of language.
Positive - Article content (1)

If you read the articles entirely, you have a good feel for what the article is about and the tone it takes. You can also consider the important information necessary for the appropriate keywords.
Negative - Problem in headline generation (3)

Many of the article headlines, especially in the beginning, covered the article topic. However, some articles towards the end only covered a paragraph of the article and not the overall topic.

Most of the time there was a clear 'best' answer, however sometimes even the 'best' one had problems. Several times none of them were very good, several times more than one would work, depending on the desires of the specific newspaper. Once there was only one option. However, since the titles were auto-generated and I had to simply pick one from a list, the task was pretty easy.

It was easy to create most headlines for the articles. The few difficult ones were due to multiple stories or themes in one single article. The headlines couldn't capture these multiple stories/themes accurately.
Negative - Problem of article (1)

The difficulty was in discerning the important context from the article.

==> Results/Task-diff-thematic/con2.tex <==
Con 2
Positive - Full generator (keywords + headlines) (6)

It was pretty easy to work with the headline system because after selecting the keywords that I thought were most important, the headlines were all created for me. All I had to do was select the points that I thought were most critical.

This simplified it by narrowing down the options and allowing the possibility to see multiple headlines that could potentially work.

P23: The main points were combined into an easy-to-use database for selection.

It was very simple to select key words, and then evaluate the presented options for headlines.

The generator put together what I was thinking most of the time.

It made the process sumple

Positive - Keywords generation (1)

P27: The site helped find the key words for the headlines.

Negative - Problem in headline generation (3)

P28: The process itself allowed for the easy creation of headlines. The difficulty arose in issues with some buttons not populating properly or some headlines missing words.

Some keywords created didn't make sense, but overall it was pretty simple to navigate and create the titles.

[Explicitly mention the need of post-editing] It wasn't difficult to generate headlines, but not every suggestion was the best choice. If I wanted to tweak or edit a headline I could not, I had to pick the following best headline.

==> Results/Task-diff-thematic/con3.tex <==
Con 3

Positive - Full generator (keywords + headlines) (5)

I think some of the wording could have been tightened to better suit the article, but there were usually 2 good options per prompt

P32: I disagree because I think the system did a good job at writing most of the headline for you based on the information you provided.

P33: [mention post-editing] super easy and efficient as well as cutting time down and being able to edit the headlines generated makes the process more meaningful Aswell.

P34: I didn't find it difficult to find the main subject and message of the articles.

P35: I found it was quite easy to create headlines, and the system was largely accurate in highlighting important information into headline format.

Negative - Problem in full generator (keywords + headlines) (5)

P36: Some were very easy and usable as presented. Others were not. For a few, the headlines based on keywords were almost unusable.

P37: Generated headlines guided content and required minimal edits in most instances. However, some articles with political nuance generated inaccurate headlines stating agreements reached that had not been requiring a close attention to detail.

P38: The system gives good ideas on how to start an article. The system does have a few confusing points though.

P39: Some seemed spot on and others seemed chaotic. But with a few tweaks, it was easy to create a headline. Some of the keywords suggested seemed totally unnecessary. The keywords were the weakest part of the system in my opinion.

P40: Some of the headlines were easy to create, and others were difficult. For the ones that were difficult, my biggest problem was choosing keywords that were actually the blatant keywords that I wanted to use. And sometimes the system came up with headlines that weren't related to the keywords I asked for.

==> motivation.tex <==
\section{Motivation}
Previous work on news generation and personalized summarization mainly focused on algorithms, so there is a need for an in-depth study the user experience (task difficulty, task satisfaction, trust on AI, control on AI) of editors on writing personalized news headlines
GPT-3 is promising in high-quality summarization with relatively small-scale text data (~3000 words), which matches the scale of single news article well; GPT-3 could do zero-shot learning and few-shot learning (the original news headline could be used as example for few-shot learning)
Currently news media also leverages data analytics to write and test headlines - write many headlines and then do A/B testing to decide the winner; so assist editors with AI to write headlines also fit that real-world workflow well
Filtering unwanted AI-generated results such as incomplete headlines and click-bait headlines with human intervention
Gap in the CHI community: to the best of our knowledge, no work on generating news headlines in CHI community for the recent 10 years, and no work on the user (editor) experience on AI-powered interactive headline generation

\section{Contribution}
Based on five human-AI interactions in text generation (Cheng et al., NACCL 2022), investigate three human-AI interactions - (1) guiding model output, (2) selecting or rating model output, and (3) post editing  - in a specific task setting of text summarization - editors writing news headlines
Propose a “double diamond” pipeline inspired by the Double Diamond design approach to help human interact with language model to come up with headlines for news articles
[Algorithm] Study the capabilities of GPT-3, a state-of-the-art language model, in determining the keywords/perspectives of news articles and generating headlines corresponding to keywords selected by users; improve the keywords and headlines generated by language models with various prompt programming and zero-shot learning
[System] Build an interactive real-time headline generator, which could be adopted to other interactive writing needs such as generating personalized news headlines for end users
[User experience] Conduct the first holistic human study on interactive headline generation system; systematically evaluate user experience; fill in the gap of previous work on headline generation and personalized text summarization

\section{Conditions for user evaluation}
1. Baseline (headlines written by professional editors) [eval only]
2. Manual (write headline without assistance)
3. GPT-3 generates a headline without any human interaction [eval only]
4. GPT-3 generates a top headline and user chooses best
5. interactive system for generating headline (perspective + choose best)
6. Interactive system: perspective + choose best + post-editing

Condition 2, 4, 5, 6 need human study as described in Human Studies section

Tutorial of writing news headlines
What is a good headline?
“TACT test”: Taste-Attractiveness-Clarity-Truth
\textbf{Taste}: Is it in good taste? Is there anything possibly offensive in the headline? Can anything in the headline be taken the wrong way?
\textbf{Attractiveness}: Is it attractive to the reader? Can it be improved so it is more engaging and interesting, without sacrificing accuracy?
\textbf{Clarity}: Does it communicate the key points of the article? Is it clear and simple? Does it use the active voice and active verbs? Are there any odd words or double meanings that could confuse the reader?
\textbf{Truth}: Is it accurate? Are the proper words or terms from the article used in the headline? Is the headline factually correct?
Source: University of Columbia http://www.columbia.edu/itc/journalism/isaacs/client_edit/Headlines.html

Human studies

Task 
Between-subjects with four conditions
Conditions
Con 2. Manual
Con 4. GPT-3 + choose best
Con 5. GPT-3 + choose best + perspective
Con 6. GPT-3 + choose best + perspective + post-editing

RQs
- RQ1 - how does human performance compare among the four interactive conditions and to the AI-generated headline or the ground truth (original) headline?
    - Quality - evaluated with a second set of participants (audience): Taste; Attractiveness; Informativeness; Truthfulness
    - Efficiency - time spent
- RQ2 - how does user experience compare for the interactive conditions: control, satisfaction and trust of AI?
    - How does perceived general satisfaction and workload compare for all conditions?

Hypotheses
- Performance: efficiency, quality (attractiveness/truthfulness/informativeness)
    - Efficiency: manual will be slower than the assisted conditions however, the more interactive conditions will decrease efficiency (e.g., condition 4 will write headlines faster than those in condition 6)
    - Quality: 
        - More interactive headline generation with perspectives will increase the attractiveness without compromising informativeness and truthfulness.
        - Previous hypothesis: Con 1 (original headline) = Con 6 (human guidance, selection and post-editing) >= Con 5 (human guidance and selection) >= Con 4 (only selection) >= Con 3 (no human intervention) > Con 2 (manual); GPT-3 conditions might outperform Con 1 (original headlines)
- User experience
    - Trust on AI (in condition 4, 5, 6): Con 6 (human guidance, selection and post-editing) > Con 5 (human guidance and selection) > Con 4 (only selection)
    - Control on AI - likert scale: exclude Con 2 (manual); Con 6 (human guidance, selection and post-editing) > Con 5 (human guidance and selection) > Con 4 (only selection)
    - Workload: Con 2 (manual) > Con 6 (human guidance, selection and post-editing) > Con 5 (human guidance and selection) > Con 4 (only selection)

Measures
[note: these measures are out of date from what is in the system interface]
Performance
- Generated headline quality (evaluated with a second set of participants) for Taste, Attractiveness, Informativeness, and Truthfulness
- Efficiency - time spent writing the headline
    - How much time they spent on each sub-task: 
        - reading news (time between starting reading and clicking “continue to write headline”
        - [primary efficiency measure] Con 2/4/5/6: writing headlines (time between clicking “continue to write headline” and clicking “submit headline”)
        - Con 5/6: selecting keywords (time between showing keywords and clicking “generate headline”)
        - Con 4/5/6: selecting headlines (time between showing headlines and clicking “sub headline”)
        - Con 6: post-editing headlines (time between clicking “Edit” and clicking “Done”)

(subjective) User Experience
    - After each task
        - Task difficulty
            - How difficult was it to write this headline for the news article? (0: Very easy; 100: Very difficult)
            - NASA TLX slider after each headline writing task
    - Post-study survey
        - Task difficulty
        - Control of AI 
        - Trust of AI 

Evaluation
Ranking: each participant sees 6 headlines for an article and ranks them
Use upwork (a distinct set of users)

Data
- Yahoo! News is the most popular news website in US (Q1 2022)
- 20 recent news (in Jun 2022) are curated over four news categories (World Politics, COVID-19, Climate Change, Science) to provide a real-world setting; US politics are avoided
- Word counts are from 300 to 1000
Headline generation with GPT3

Procedure
- Step 1: consent form
- Step 2: summary instructions
- Step 3: detailed instructions, criteria, and examples
- Step 4: practice with 2 articles, will indicate that’s practice
- Step 5: task
    - Each participant writes headlines for 20 randomized news articles in one of the above conditions: 
    - They will first read the article and then write the headline
    - Con 2. Manual: Participants will read the article and write the headline without any assistance.
    - Con 4. GPT-3 + choose best
    - Con 5. GPT-3 + choose best + perspective
    - Con 6. GPT-3 + choose best + perspective + post-editing
- Step 6: User-exit survey

Recruitment plan & budget
- User study: 
    - Participants: 40 participants, 10 participant for each condition
    - Each participant will write headlines for 2 (practice) + 20* (task) articles per participant, 1 hour, 20 for each participant
Budget: 21.9*40 in total
    - End up with 800 headlines in total (200 headlines per condition, 40 headlines per article)
OpenAI GPT3 API: 1 condition with 1 run per article x 20 articles x 10 participants + 2 condition with 2 run per article x 20 articles x 10 participants + 1 condition x 1 run per article x 20 article = 1020 runs (minimum); ~\$0.06 for each run, ~\$60 in total
We hope to have some extra budget to run API just in case e.g. participant refreshes / drops

==> sections/discussion-prev-1.tex <==
\section{Discussion}
\label{sec:discussion}
\subsection{Summary and interpretation of findings}

We investigated how different forms of AI assistance for writing news headlines affect headline quality (RQ1), effort (RQ2), and perceptions of control and trust (RQ3). 
%
Regarding task quality, \textit{GPT only} produced the best headlines, on average, while participants writing manually did the worst. 
%
While this might suggest automatic methods are sufficient for headline generation; importantly, the \textit{GPT only} headlines were not perfect, and still ranked last in some cases.
%
Human control is needed to edit and make the final say in case of system error.
 %\textit{Guidance + Selection} and \textit{Guidance + Selection + Post-editing} %generated similar number of top-ranked headlines, but \textit{Guidance + Selection} and \textit{Guidance + Selection + Post-editing} produced more bottom-ranked headlines. 
%It might be due to a discrepancy of criteria and focus to evaluate headlines, even implicit bias between human editors and evaluators. 
%Another possibility was that the headlines generated in \textit{GPT only} were better than headlines offered previous to human selection. 
Of the assisted methods, guiding model output (using keywords) helped to generate better headlines than selection alone, and  human post-editing was not required for achieving high quality in the headline generation task. 
%
Further, interactions with less control were the fastest. Writing headlines (post-edit and manual conditions) took longer compared with only guiding the model and selecting from generated headlines.
%
Meaning, that when control is desired, supporting selection or guidance can yield high-quality headlines quickly, particularly when the original model outputs are good. 
%
Post-editing would likely be more critical had the model quality been lower.
%

%
Surprisingly, we found no significant differences between conditions for any of the subjective measures---task difficulty, control, or trust---even though the conditions varied in terms of required effort and control. 
%
For example, simply selecting choosing one of the system-generated headlines  affords far less control (and takes less effort) than writing a headline from scratch. 
%
As discussed in Section~\ref{sec:results_control}, this could be due to the measure (e.g., that all participants felt they had some influence over the final headlines). 
%
Another possible reason is due to the high quality of the model outputs. Participants were generally happy with the model headlines from which they could select. And, they did not need to do much editing (or have additional control) in those conditions.
%on AI did not differ between conditions, even though the conditions varied in terms of required effort and level of control.

% \subsection{Implications for human intervention on AI-generated contents}
%\alison{We should compare our results to prior work (like Viv's study and earlier works on machine translation) that find post editing is REALLY important (because AI outputs are not great), we should discuss how we found that GPT-3 headlines were high quality, which means that post editing/control was not required to improve the headlines (at least on average), but that control is still important since human needs to have the final say (e.g., even if AI only makes a few mistakes, they could be really bad) - this is something good for the discussion but we might also mention earlier that we expected human or AI + human to do a *better* job (based on prior interactive NLP works)}
% \subsubsection{When human intervention is needed for AI-generated content, and what kind of intervention is needed}
\label{sec:implications}

% Interestingly, \textit{GPT only} outperformed the assisted methods in terms of headline quality, which is counterintuitive to earlier findings that human intervention is required to improve the quality of AI-generated text contents. For example, Lai et al. \cite{laiExplorationPostEditingEffectiveness2022}) demonstrated the importance of post-editing for text summarization tasks.\joel{but did Lai et al. use LLMs?  Is it possible that the models are just that good for this task now?  It might make sense since they have seen probably millions of headlines;  random question - is it possible that GPT3 was trained on any of the news articles in the study?  Or was this after GPT3 was released?  }
%
% As our system-generated headlines were high-quality, on average, editing was not necessary to improve performance.
%
% However, the system outputs were not perfect. And humans, not AI, are held \textit{accountable} for mistakes in the final output. 
%Although a within-subjects study might have better highlighted experience differences, the results headline creation task suggests that LLMs hold a strong promise for intensive, succinct and concrete text generation tasks and human editors do not see a necessity to change or tweak the output of AI. If AI-generated outputs were unsatisfactory which were common in previous work not using LLM \cite{laiExplorationPostEditingEffectiveness2022}, more intensive human control methods such as post-editing would be necessary for guaranteeing the quality of final artifacts. 
% In such AI-assisted generation cases where human control is desired, or when humans are the consumers instead of the producers of text and want to control the information they receive, human guidance and selection without post-editing is appropriate. 
%
% Post-editing is needed only when model outputs are particularly low quality. 

% Further, for creative and open-ended tasks, human involvement might be more valuable and meaningful. For example, one participant commented, ``I could see how this would be beneficial in situations where time is limited, but it does not replace the creativity and reasoning a human has.'' 
We also expect that more human intervention is needed to guide or restrict LLM outputs in other settings. For example, information workers can leverage LLMs for efficient parallel prototyping \cite{dowParallelPrototypingLeads2010}: humans can propose a diverse set of potential directions to guide AI exploration, and then select or rate AI-generated content.
%
Here humans are likely to have stronger preferences for guiding and judging system outputs.

% \subsubsection{Ethical concerns of over-reliance on AI-generated contents}

%Although we have observed that the performance of headlines generated in \textit{GPT only} was even comparable to \textit{Baseline} and the headlines in \textit{GPT only} did not demonstrate evident biases or ethical issues, 
% While we did not observe any biases or ethical issues in the headlines generated by \textit{GPT-3} in our study, there is an open question of to what extent AI should be relied upon. Shneiderman proposes that ``we should reject the idea that autonomous machines can exceed or replace any meaningful notion of human intelligence, creativity, and responsibility'' \cite{shneiderman2022human}. 
%
% We echo that AI should not be relied upon entirely for creating text.%, even in less-critical domains like news headlines.%\joel{not a good idea to call this less critical where in the beginning of the paper there is a lot of discussion on how important they are.  Also bad headlines can lead to misinfo.  I know what you're getting at but it should be reframed} 
% It is important for human experts to use their expertise and judgment when working on content generation with AI and ensure that the content produced is fair, ethical, and aligned with societal values.

% \subsection{Limitations}
%\alison{its important to tie the limitations to the results, meaning, how might they affect how our results can generalize? or for each limitation, what does it mean for how we should interpret the results.. for example, you say that the time budget made people work quickly which limits their creativity.. what does this mean? that had participants had more time, they might have written *better* headlines than the AI? or that our results might not generalize to writing tasks where speed is not important?}

% \subsubsection{Limitations of human study design}

% unrealistic time constraint
%Due to time and budget limitation, 
% Each participant took one hour to read 20 news articles and generate 20 news headlines in the user study, which was doable but intensive, especially for \textit{Manual only} condition without AI assistance. The task intensity might harm the creativity of humans, which requires flexibility and time \cite{nijstadDualPathwayCreativity2010, zabelinaCreativityFlexibleCognitive2010}.
%
Had we given more time for the task, participants writing headlines manually may have performed better.
% participant expertise
And, although the participants had editing and writing backgrounds and instructions for writing good news headlines were provided to them, those participants were not professional news editors with solid editing training. This put the participants writing headlines manually at a further disadvantage compared to the AI-assisted conditions.
% \joel{I agree with this...we don't have professional headline writers and that might actually be why GPT3 seems to be the best}
%
Future work could explore how professional news editors perform in this task setting.
%We are interested in how professional news editors would perform in this task setting, and one possible direction for future work is expert supervision in AI-assisted text generation. 
% comparison
Finally, we performed a between-subject study, not a within-subjects, so there was a lack of direct comparison between different human-AI conditions: for example, \textit{Manual only} participants were not aware of how AI assistance could help with the task, and \textit{Selection} participants could not compare other methods to control AI-generated headlines.
%

\subsection{Future work}

\subsubsection{Systematic evaluation on expert intervention for LLM-generated contents} As discussed in Section \ref{sec:implications}, it might be infeasible to fully automate highly creative and open-ended content creation tasks, e.g., writing a compelling piece of fiction or a rigorous scientific paper. Those tasks require a holistic overview, skills of planning and reasoning, and domain-specific knowledge, especially subtlety and tacit knowledge
% \joel{domain is used twice in the same sentence;  unclear what the insightful overview is} 
to fully grasp the nuances and complexities of human language. Neither LLMs \cite{valmeekamLargeLanguageModels2022} nor novices \cite{sunComparingExpertsNovices2022, macneilFramingCreativeWork2021, seeComparingQualityCrowdsourced2013} have that expertise, and expert intervention is required to guide, control and tweak AI models for those types of content generation. \joel{I'd be wary of a reviewer saying ChatGPT can write great stories..and it kind of can}
%
There exist some proofs-of-concept for how LLMs could assist experts in those creative and open-ended tasks \cite{yuanWordcraftStoryWriting2022a, berkovskyHowNovelistsUse2018, freiknechtProceduralGenerationInteractive2020,yangAIActiveWriter}. Yet more systematic evaluations are needed to probe the capabilities of LLMs and benchmark quality, efficiency, and user perception.

% \subsubsection{Indirect human control for personalized content generation}

%As reflected by the headline quality results, 
% Headline creators and evaluators might not have consistent perspectives or preferences, as reflected by quality rating mismatches. For example, some headlines chosen as best by study participants were ranked low by evaluating annotators.%, which could result in human-selected headlines with low rankings from evaluators. 
% If the difference between content creators’ and consumers’ preferences cannot be mitigated, one option to improve consumers’ ranking is to transfer the control to consumers. 
% \alison{i'm trying to edit but its not clear to me the point of this next bit.. something about how we let consumer control but this is veering a bit far away from what we studied - maybe drop this one}
% For example, Horvitz proposed balancing autonomous actions with direct manipulation in his formative paper on mixed-initiative systems \cite{horvitzPrinciplesMixedinitiativeUser1999}. Besides direct control or manipulation, indirect control with end-users’ contextual information might also be valuable for AI-generated content for low effort and truthful data. User history is a potential resource for end-user preferred perspectives, and AI can use that contextual information of end-users to personalize the content for the audience.

\subsubsection{Opportunities for prompt learning paradigms and prompt designs}
Our study focus was on AI-assisted news headline generation, and not on comparing the performance of different prompt learning paradigms and prompt designs. We directly used the zero-shot prompt learning paradigm for LLMs for headline generation. However, there are more possibilities with one-shot or few-shot learning paradigms: examples can be crafted for different types of news articles. 
Future work should explore these varied methods.
%Besides, three headlines were generated by GPT-3 in one round for human selection in all human conditions with selection interaction, while only one headline was generated for each article in one round for \textit{GPT only}. That inconsistency could influence the headlines generated previous to human selection. It suggests that future work could take prompt designs into human-AI interaction of LLM-based text generation, such as how to match prompt designs with interaction types, and whether humans could change or tweak prompts fed into LLMs.

\section{Conclusion}
% \alison{if there is space and time, it's nice to end with a succinct conclusion}
Human-AI text co-creation has received growing attention along with the advancement of LLMs. %\joel{not sure what this first sentence is saying.  ALso no need to say what LLMs say at this point.  }
However, there is a lack of systematic evaluation of performance and experience among different types of human-AI interaction for text generation tasks. We explore human-AI interaction through the lens of News Headline generation and compare three common types of human-AI interactions for text (guiding model outputs, selecting from model outputs, and post-editing) with human-only and AI-only methods. We first developed an LLM-powered headline generation system and invited 40 participants with editing backgrounds for a user study. We then recruited 20 expert evaluators to rate the headlines generated by the six methods. 
The LLM alone can generate satisfactory news headlines, on average, but human control is needed to fix undesirable model outputs.
% particularly when due to bias or promoting misinformation.
%
Of the interaction methods, guiding model output added the most benefit with the lowest cost (in time and effort). Post-editing was not needed as model outputs were fairly high quality, to begin with.
%
Further, AI assistance did not harm participants’ perception of control compared to freeform editing. 
%We extended those results to future work for different AI-assisted text generation scenarios.
%\joel{this conclusion needs way more punch.  Highlight what was surprising and why. And be explicit about what this means for the field.}
%\joel{Let me play devil's advocate: one could takeaway that human-AI collaboration may not be necessary.  Just use the LLM since it will be faster and is actually higher quality even if it gets a few things wrong here and there.  Is that the message one wants to send? }

==> sections/discussion-prev-2.tex <==
\section{Discussion}
\label{sec:discussion}
\subsection{Summary and interpretation of findings}

We investigated how different forms of AI assistance for writing news headlines affect headline quality (RQ1), effort (RQ2), and perceptions of control and trust (RQ3). 
Regarding task quality, \textit{GPT only} produced the best headlines, on average, while participants writing manually did the worst. 
While this might suggest automatic methods are sufficient for headline generation; importantly, the \textit{GPT only} headlines were not perfect, and still ranked last in some cases.
Human control is needed to edit and make the final say in case of system error.
Of the assisted methods, guiding model output (using keywords) helped to generate better headlines than selection alone, and  human post-editing was not required for achieving high quality in the headline generation task. 
Further, interactions with less control were the fastest. Writing headlines (post-edit and manual conditions) took longer compared with only guiding the model and selecting from generated headlines.
Meaning, that when control is desired, supporting selection or guidance can yield high-quality headlines quickly, particularly when the original model outputs are good. 
Post-editing would likely be more critical had the model quality been lower.

Surprisingly, we found no significant differences between conditions for any of the subjective measures---task difficulty, control, or trust---even though the conditions varied in terms of required effort and control. 
For example, simply selecting choosing one of the system-generated headlines  affords far less control (and takes less effort) than writing a headline from scratch. 
As discussed in Section~\ref{sec:results_control}, this could be due to the measure (e.g., that all participants felt they had some influence over the final headlines). 
Another possible reason is due to the high quality of the model outputs. Participants were generally happy with the model headlines from which they could select. And, they did not need to do much editing (or have additional control) in those conditions.

\label{sec:implications}

We also expect that more human intervention is needed to guide or restrict LLM outputs in other settings. For example, information workers can leverage LLMs for efficient parallel prototyping \cite{dowParallelPrototypingLeads2010}: humans can propose a diverse set of potential directions to guide AI exploration, and then select or rate AI-generated content.
Here humans are likely to have stronger preferences for guiding and judging system outputs.

Had we given more time for the task, participants writing headlines manually may have performed better.
And, although the participants had editing and writing backgrounds and instructions for writing good news headlines were provided to them, those participants were not professional news editors with solid editing training. This put the participants writing headlines manually at a further disadvantage compared to the AI-assisted conditions.

Future work could explore how professional news editors perform in this task setting.

Finally, we performed a between-subject study, not a within-subjects, so there was a lack of direct comparison between different human-AI conditions: for example, \textit{Manual only} participants were not aware of how AI assistance could help with the task, and \textit{Selection} participants could not compare other methods to control AI-generated headlines.


\subsection{Future work}

\subsubsection{Systematic evaluation on expert intervention for LLM-generated contents} As discussed in Section \ref{sec:implications}, it might be infeasible to fully automate highly creative and open-ended content creation tasks, e.g., writing a compelling piece of fiction or a rigorous scientific paper. Those tasks require a holistic overview, skills of planning and reasoning, and domain-specific knowledge, especially subtlety and tacit knowledge to fully grasp the nuances and complexities of human language. Neither LLMs \cite{valmeekamLargeLanguageModels2022} nor novices \cite{sunComparingExpertsNovices2022, macneilFramingCreativeWork2021, seeComparingQualityCrowdsourced2013} have that expertise, and expert intervention is required to guide, control and tweak AI models for those types of content generation. \joel{I'd be wary of a reviewer saying ChatGPT can write great stories..and it kind of can}
%
There exist some proofs-of-concept for how LLMs could assist experts in those creative and open-ended tasks \cite{yuanWordcraftStoryWriting2022a, berkovskyHowNovelistsUse2018, freiknechtProceduralGenerationInteractive2020,yangAIActiveWriter}. Yet more systematic evaluations are needed to probe the capabilities of LLMs and benchmark quality, efficiency, and user perception.

\subsubsection{Opportunities for prompt learning paradigms and prompt designs}
Our study focus was on AI-assisted news headline generation, and not on comparing the performance of different prompt learning paradigms and prompt designs. We directly used the zero-shot prompt learning paradigm for LLMs for headline generation. However, there are more possibilities with one-shot or few-shot learning paradigms: examples can be crafted for different types of news articles. 
Future work should explore these varied methods.

\section{Conclusion}
Human-AI text co-creation has received growing attention along with the advancement of LLMs.
However, there is a lack of systematic evaluation of performance and experience among different types of human-AI interaction for text generation tasks. We explore human-AI interaction through the lens of News Headline generation and compare three common types of human-AI interactions for text (guiding model outputs, selecting from model outputs, and post-editing) with human-only and AI-only methods. We first developed an LLM-powered headline generation system and invited 40 participants with editing backgrounds for a user study. We then recruited 20 expert evaluators to rate the headlines generated by the six methods. 
The LLM alone can generate satisfactory news headlines, on average, but human control is needed to fix undesirable model outputs.
Of the interaction methods, guiding model output added the most benefit with the lowest cost (in time and effort). Post-editing was not needed as model outputs were fairly high quality, to begin with.
Further, AI assistance did not harm participants’ perception of control compared to freeform editing. 

==> sections/introduction-prev-1.tex <==
\section{Introduction}

\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{figures/Teaser.png}
    \caption{Human-AI interactions for text generation can fall within a range of no human control effort (AI-only) to full human control effort (manual methods).  %Spectrum of human control on human-AI co-created contents.
}
\label{fig:teaser}
\end{figure*}
% \alison{were still intermixing 'ai-assisted' and 'human-ai co-creation' - does anyone prefer one over the other? i've been tending to 'human-ai co-creation' but would be fine with either}
% \ja{I also lean towards 'human-ai co-creation' as it emphasized both human and AI}
% \joel{my take is did we check to see if someone has already used a term for this? I think AI-assisted might be more common.  }
Human-AI text co-creation, a collaborative process where humans and artificial intelligence systems work together to generate text, has promising applications, such as summarization \cite{chintaguntaMedicallyAwareGPT32021, goyalNewsSummarizationEvaluation2022, zhangBenchmarkingLargeLanguage2023, bhaskarZeroShotOpinionSummarization2022}, creative writing \cite{clarkCreativeWritingMachine2018, yuanWordcraftStoryWriting2022a, roemmeleWritingStoriesHelp2016}, and data-backed text generation \cite{strobeltGenNIHumanAICollaboration2022}.
Recent advances in large language models (LLMs), including Generative Pre-trained Transformer (GPT) \cite{brownLanguageModelsAre2020}, demonstrate a previously unmatched ability to generate human-like text \cite{bommasaniOpportunitiesRisksFoundation2021}. 
In fact, the performance of task-agnostic LLMs had surpassed that of other state-of-the-art task-specific models in various natural language processing (NLP) tasks \cite{leeCoAuthorDesigningHumanAI2022a}.  
%LLMs 
% quality is improving (on average), but systems still make mistakes
Yet, LLM-backed systems are not perfect, they suffer from hallucinations, bias, and sometimes generate inappropriate or inaccurate artifacts such as toxic, discriminatory and false information \cite{wangExploringLimitsDomainAdaptive2022, jakeschCoWritingOpinionatedLanguage}.
% further, AI cannot be accountable, so humans need control/oversight
Further, AI lacks \textit{accountability} \cite{shneiderman2022human}, meaning the responsibility falls to humans when mistakes are made in human-AI text co-creation.

% PARA 2: 
% AI-assisted text generation is not new, but we still lack understanding of tradeoffs between control/effort - no systematic evaluation of common interaction forms
% research goals
%Those emerging technologies prompts us to reconsider the 
Thus, we explore human-AI text co-creation from two perspectives. First, how can humans best leverage LLMs in writing tasks---in terms of quality and effort? And, second, how does interacting with these models affect humans' sense of ownership and system trust while performing their tasks?  \joel{this para and the one above need a better segue/transition. }


% interaction types
Humans can interact with AI for writing tasks in many ways, which vary in terms of human control. For example, Cheng et al. \cite{chengMappingDesignSpace2022} identified common human-AI interactions for text summarization, including guiding model output, selecting from model outputs, and post-editing. However, these interactions have not been evaluated systematically. 
%
% study task
We studied these common interaction types in the context of LLM-assisted news headline writing: \textit{guidance} for the LLM headline generation with perspectives (keywords or facets), \textit{selection} from three LLM-generated headlines, and \textit{post-editing} the LLM-generated headline. 
%
We chose the task of writing news headlines, because it is a representative text summarization task that is accessible and simple compared with more demanding content creation tasks, such as free-form creative writing or long-form summarization (e.g., writing paper abstracts). And a study using the headline generation task has the potential to spawn research in more complex areas of human-AI collaboration.
%
%\alison{I'm introducing this tradeoff bit here.. not sure if we want to push on that or not but if we do needs to come up earlier in the motivation.. i'll come back to this}
We compared headline quality, efficiency, and user experience for headlines written by AI, fully manually, or aided by one of three human-AI system variants---ranging from minimal oversight to heavy intervention: (1) \textit{selection}, (2) \textit{guidance + selection}, (3) \textit{guidance + selection + post-editing} (Figure \ref{fig:teaser}). 
% Results and Contributions
% \alison{this needs a little more detail of the results - think about what are the key points we want future researchers or creators of LLM-assisted writing agents to take away from this..}
Results showed that the LLM alone generated the highest quality headlines, on average, but also produced sub-optimal headlines in some cases. Practitioners must decide if such errors are acceptable given their needs.  %demonstrating its potential for assisting the news headline generation process,
%
Of the AI-assisted generation settings, both \textit{selection} and \textit{guidance + selection} yielded high-quality headlines faster than when human writing intervention was required (i.e., post-editing or manual).
% \joel{I think this gets really detailed.  Unless you are familiar with the Cheng paper you have to guess what guidance and selection mean.  I would say you can either 1. not list the takeaways or 2. keep it more general without going into the terminology.}   }
%and assistance of LLM without post-editing interaction can significantly increase the efficiency of headline creation without sacrificing human’s level of control.
%
%
% illustrates these study conditions on the human control spectrum. 
% \alison{do we consider the system implementation to be a contribution? could we open source it? -- that's a question for Joel/Alex}
% \joel{if they're just the out of the box methods, then no.}

%1) between AI-only and human-AI: how does quality compare for contents generated by LLM-only and by humans with LLM assistance; and 2) within human-AI: which LLM-assisted method is more effective, efficient and user-friendly?
% While AI can never be truly accountable \cite{shneiderman2022human}, it encourages us to reconsider how much human effort or control is optimal for those emerging text generation technologies in terms of task quality, efficiency as well as user experience. 

% motivation - AI-assisted text summarization
%To deepen our understanding of how LLM could assist human for content creation, we chose to study text summarization, a representative text generation task for its accessible and low-weight nature compared with relatively demanding content creation tasks such as writing a paper or article. 
%Cheng et al. \cite{chengMappingDesignSpace2022} conducted a systematic literature review on AI-assisted text summarization and identified several types of human-AI interactions in this context, including guiding model output, selecting or rating model output and post-editing. 
% They followed up the review with a formative study on those interactions using Wizard-of-Oz techniques and found that humans may desire control on AI-generated text such as “final say” when they are using the output \cite{chengMappingDesignSpace2022}. Moreover, AI algorithms such as LLMs might not have the same level of understanding and context as humans, and therefore might generate inappropriate or inaccurate artifacts such as toxic, discriminatory and false information \cite{wangExploringLimitsDomainAdaptive2022, jakeschCoWritingOpinionatedLanguage}. There are where human control, guidance, and oversight could play a role in the co-summarization process, while the formats and levels of human involvements highly depend on the context.
% It prompts us to ask three research questions: how different types of human control affect AI-assisted text summarization in terms of task quality (RQ1), efficiency (RQ2), and human experience (RQ3), compared to fully manual or fully automatic approaches. 
% \RQO\space and \RQT
% experiment - task, interactions
% To answer those three RQs, 
%We extended their work with a human study of a functional system based on LLMs, and selected news headline generation, a typical text summarization task requiring both accuracy and creativity and used in previous work of studying the capability of LLM for text summarization \cite{goyalNewsSummarizationEvaluation2022}, as a testbed. Our study was based on two research questions (RQs): \RQO\space and \RQT\space

%In order to answer those two RQs, we generated headlines using a few hybrid approaches with different types of human control: 1) guiding the LLM-generated headlines with perspectives (keywords or facets), 2) selecting the LLM-generated headlines , and 3) post editing of LLM-generated headlines. 

%We then compared the quality of those headlines with manual-only or AI-only baselines: 1) original news headlines (manual-only), 2) manually written headlines by participants (manual-only), 3) LLM-generated headlines (AI-only). We also measured the efficiency and user experience of those human-AI hybrid approaches for headline generation. 




==> sections/introduction-prev-2.tex <==
\section{Introduction}

Human-AI text co-creation, a collaborative process where humans and artificial intelligence systems work together to generate text, has promising applications, such as summarization \cite{chintaguntaMedicallyAwareGPT32021, goyalNewsSummarizationEvaluation2022, zhangBenchmarkingLargeLanguage2023, bhaskarZeroShotOpinionSummarization2022}, creative writing \cite{clarkCreativeWritingMachine2018, yuanWordcraftStoryWriting2022a, roemmeleWritingStoriesHelp2016}, and data-backed text generation \cite{strobeltGenNIHumanAICollaboration2022}.
Recent advances in large language models (LLMs), including Generative Pre-trained Transformer (GPT) \cite{brownLanguageModelsAre2020}, demonstrate a previously unmatched ability to generate human-like text \cite{bommasaniOpportunitiesRisksFoundation2021}. 
In fact, the performance of task-agnostic LLMs had surpassed that of other state-of-the-art task-specific models in various natural language processing (NLP) tasks \cite{leeCoAuthorDesigningHumanAI2022a}.  

Yet, LLM-backed systems are not perfect, they suffer from hallucinations, bias, and sometimes generate inappropriate or inaccurate artifacts such as toxic, discriminatory and false information \cite{wangExploringLimitsDomainAdaptive2022, jakeschCoWritingOpinionatedLanguage}.

Further, AI lacks \textit{accountability} \cite{shneiderman2022human}, meaning the responsibility falls to humans when mistakes are made in human-AI text co-creation.

Thus, we explore human-AI text co-creation from two perspectives. First, how can humans best leverage LLMs in writing tasks---in terms of quality and effort? And, second, how does interacting with these models affect humans' sense of ownership and system trust while performing their tasks?

Humans can interact with AI for writing tasks in many ways, which vary in terms of human control. For example, Cheng et al. \cite{chengMappingDesignSpace2022} identified common human-AI interactions for text summarization, including guiding model output, selecting from model outputs, and post-editing. However, these interactions have not been evaluated systematically. 

We studied these common interaction types in the context of LLM-assisted news headline writing: \textit{guidance} for the LLM headline generation with perspectives (keywords or facets), \textit{selection} from three LLM-generated headlines, and \textit{post-editing} the LLM-generated headline. 

We chose the task of writing news headlines, because it is a representative text summarization task that is accessible and simple compared with more demanding content creation tasks, such as free-form creative writing or long-form summarization (e.g., writing paper abstracts). And a study using the headline generation task has the potential to spawn research in more complex areas of human-AI collaboration.

We compared headline quality, efficiency, and user experience for headlines written by AI, fully manually, or aided by one of three human-AI system variants---ranging from minimal oversight to heavy intervention: (1) \textit{selection}, (2) \textit{guidance + selection}, (3) \textit{guidance + selection + post-editing} (Figure \ref{fig:teaser}). Results showed that the LLM alone generated the highest quality headlines, on average, but also produced sub-optimal headlines in some cases. Practitioners must decide if such errors are acceptable given their needs. Of the AI-assisted generation settings, both \textit{selection} and \textit{guidance + selection} yielded high-quality headlines faster than when human writing intervention was required (i.e., post-editing or manual).

\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{figures/Teaser.png}
    \caption{Human-AI interactions for text generation can fall within a range of no human control effort (AI-only) to full human control effort (manual methods).
}
\label{fig:teaser}
\end{figure*}

==> sections/methods-prev-1.tex <==
\section{Evaluating AI-assisted news headline generation}
% \joel{there needs to be a better transition from the end of Section 2 to the beginning of Section 3.  }
Our study focused on three research questions (RQs): \textbf{RQ1}: How do different forms of assistance affect quality? Is AI alone good enough or is human input needed for high quality?
\textbf{RQ2}: How do different forms of assistance affect effort (task time and perceived difficulty)? \textbf{RQ3}: How do different forms of assistance affect feelings of ownership (perceived control) and trust? 
%
To answer those RQs, we explored how three variants of AI-assisted news headline generation affect headline quality (RQ1), effort (RQ2), and sense of ownership and trust (RQ3), compared to fully manual or fully automatic approaches.
% \joel{for each of the RQs - leave it "compared to fully automatic and fully manual" and say we compare them to fully automatic and manual approaches at the end of the paragraph.  Right now it is an awkward read} 
%To answer \RQO\space and \RQT, we design a between-subjects study of AI-assisted news headline generation with three conditions, and compared the results with three baseline conditions.

\subsection{Task and data}
We chose to study AI-assisted text generation in the context of news headline generation due in part to the task familiarity---news is an accessible text domain and many already have a sense of what makes a good (or bad) news headline. Further, writing high-quality news headlines requires a balance of creativity and accuracy beyond simple text summarization, yet takes less time and effort than long-form summarization, such as writing paper abstracts or news article summaries. 
%Creativity and the ability to craft an appealing and concise message is key to attract readers to the article. Accuracy and brevity is also critical for truthfully reflect the content of the article and avoid creating “click-baits” and missing information. 
Finally, news headlines are easier to evaluate than more open-ended or longer-form content generation tasks.

%, as the resource of recent news articles. 
We curated 20 recent news articles (in June 2022) over four news categories (World Politics, COVID-19, Climate Change, Science), all  popular, well-known topics at that time.\footnote{The chosen articles ranged from 300 to 1000 words.} %News of US politics were avoided in case of offensive contents for certain participants. 
%Word counts of those news articles covered a wide range from 300 to 1000 words.
The articles came from Yahoo! News,\footnote{https://news.yahoo.com/} the most popular news website in US (Q1 2022).\footnote{https://today.yougov.com/ratings/entertainment/popularity/\\news-websites/all}


\subsection{AI-assisted news headline generation types and system variants}

% \joel{we need to be upfront about how many variants there are.  The bulk of this section focuses on three until the end where a fourth is mentioned out of nowhere.  Also, is there a fifth variant - fully automatic? \alison{updated re: 4 variants - the automatic one is not a studied condition (we just compare it for quality)}}

We explored four headline writing variants: writing manually or assisted by AI using one of three common human-AI interaction types identified by prior work \cite{chengMappingDesignSpace2022}:
\textit{guidance} of the LLM headline generation with perspectives (keywords or facets), \textit{selection} from three LLM-generated headlines, and \textit{post-editing} the LLM-generated headline.
%
As we are interested in understanding the  tradeoffs between control and effort in AI-assisted generation tasks, we chose to compound the different interaction types instead of exploring them separately.
%
Specifically, we developed an AI-assisted news headline generation system with four variants:
\begin{itemize}
    \item \textit{Selection}: LLM generates three headlines for each news article (\textit{generate headlines}) and the user chooses the best headline;
    \item \textit{Guidance + Selection}: LLM extracts several potential perspectives (keywords) for each news article (\textit{extract perspectives}), the user chooses one or more perspectives to emphasize in the headline, then LLM generates three headlines for each news article based on the selected perspectives (\textit{generate headlines w/ perspectives}), and, finally, the user chooses the best headline;
    \item \textit{Guidance + Selection + Post-editing}: the same as \textit{Guidance + Selection} but the user is further able to edit the chosen headline (post-editing);
    \item \textit{Manual only}: the participant writes news headline without any assistance.
\end{itemize}
%In the fourth variant, \textit{manual only}, the participant writes news headlines without any assistance.
%

\subsection{System Implementation}
The system was built on the React and Redux front-end frameworks and used Firebase real-time database to store user interaction data. We chose OpenAI's GPT-3.5 \textit{text-davinci-002} model, the state-of-the-art LLM when the study was conducted (July 2022) for the model. The frontend directly called  OpenAI's GPT-3.5 API using prompt programming (see below) to \textit{extract perspectives} (keywords) and \textit{generate headlines}---with and without supplied perspectives---and presents the results to the user (see Figure \ref{fig:interface} as an example). 
%
 %As mentioned in Section \ref{sec:studydesign}, the AI-assisted system offered four types of interactions:

% \alison{whats important about zero-shot learning here? is that one of many options we could have chosen?}
To determine the optimal prompts for \textit{extract perspectives}, \textit{generate headlines}, and \textit{generate headlines w/ perspectives} with the GPT-3.5 API, we tested several configurations, and chose the zero-shot learning paradigm (no examples of news headlines included) for broad coverage of news topics. Below are the finalized prompts for corresponding tasks:
\begin{itemize}
    \item \textit{extract perspectives}: "Please identify five keywords and key phrases (nouns) for the following news article.\textbackslash nNews article:\textbackslash n + [news article] + \textbackslash nFive keywords and key phrases (nouns), separated with comma:\textbackslash n"
    \item \textit{generate headlines}: "Please come up with three high-quality (attractive, clear, accurate and inoffensive) headlines for the following news article.\textbackslash nNews article:\textbackslash n\textbackslash n + [news article] + \textbackslash n\textbackslash nThree high-quality headlines:\textbackslash n"
    \item \textit{generate headlines w/ perspectives}: "Please come up with three high-quality (attractive, clear, accurate and inoffensive) headlines for the following news article including keyword(s): [keyword(s) selected by participants].\textbackslash nNews article:\textbackslash n\textbackslash n + [news article] + \textbackslash n\textbackslash nThree high-quality headlines:\textbackslash n"
\end{itemize}
\joel{are all these newline commands supposed to be in the above?  It looks weird.}
GPT-3.5 API takes the above prompts and returns the requested outputs.
%
To thoroughly test the reliability of LLMs, we utilized a temperature setting of 1, maximizing the variety in the output. Additionally, we set a token count of 400, ensuring an adequate allowance for both input data - comprising prompts and news articles - and output data, which included several keywords or news headlines.

\begin{figure*}
    \centering \includegraphics[width=0.6\textwidth]{figures/Interface.png}
    \caption{AI-assisted news headline generation interface for \textit{guidance + selection + post-editing} condition: (A) news reading panel, (B) perspectives (keywords) selection panel (multiple keywords can be selected), (C) headline selection panel with post-editing capability, and (D) difficulty rating slider. Note: (B), (C) and (D) are hidden from the user until the requisite step is finished (e.g., the user does not see the difficulty rating slider until after finalizing the headline). %The selected headlines would be shown on the top of news article in (A). 
    Interface variants for all study conditions can be found in the Appendix \ref{appendix:a}.}
\label{fig:interface}
\end{figure*}

\subsection{Study design}
\label{sec:studydesign}
This study consisted of two phases: (1) AI-assisted news headline generation and (2) human evaluation of the generated headlines.
%
The first phase followed a between-subjects experimental design with four conditions, from least human control to maximal human control: (1) \textit{Selection}, (2) \textit{Guidance + Selection}, (3) \textit{Guidance + Selection + Post-editing} and (4) \textit{Manual only}. In the second phase, human evaluators ranked the headlines generated in the first phase and headlines from two baseline conditions.

% \begin{figure*}
%     \centering \includegraphics[width=0.9\textwidth]{figures/Workflow.png}
%     \caption{Procedure of the user study: participants would first read the instructions on how to write high-quality news headlines, then go through the practice round with 2 news headline generation tasks and the user study with 20 news headline generation tasks, and complete the post-study survey. Screenshots for  those steps can be found in Appendix \ref{appendix:a}.}
% \label{fig:study1workflow}
% \end{figure*}

\subsubsection{Phase I: AI-assisted headline generation}\hfill\\
\newline
\noindent{\it Participants} We recruited 40 participants, 10 per condition on a freelancing platform Upwork\footnote{https://www.upwork.com/} (28 females, 11 males, 1 non-binary) who read news articles with relatively high frequency: a few times a day (29) or a few times a week (11). All of the participants had experience in journalism, editing or writing. Education backgrounds were varied: Bachelor's Degree: 18, Master's Degree: 11, Some High School or High School: 10, Prefer not to say: 1).
\\

\noindent{\it Procedure} The study participants crafted headlines for 20 articles across four distinct themes: World Politics, COVID-19, Climate Change, and Science, with each topic encompassing five articles. To prevent the possibility of eliciting negative emotional responses or influencing participant behavior, news pertaining to Domestic and US politics was purposefully omitted from the study. The overall study procedure 
% is illustrated in Figure \ref{fig:study1workflow} and 
includes a study instruction round, practice round, human study, and a post-task survey. Each participant was randomly assigned to one of the four study conditions and paid \$20 for their 1-hour participation.
% \joel{Figure 3 should be on the same page as the reference to the figure.  Right now it is two pages away.  Please fix.}

Participants first completed the \textit{study instruction}, where they learn how to use the system assigned to them with different types of AI assistance (see screenshots in Appendix \ref{appendix:a} as Figure \ref{fig:inst1} and Figure \ref{fig:inst2}). 
%
Then participants were asked to write headlines for 2 practice articles (\textit{practice round}) before moving on to the \textit{human study}, which involved writing headlines for 20 task articles.
For each article, participants first read the article and then click “Continue to Write Headline" after they finish reading.
% \alison{describe the general differences between conditions in the procedure}
Then they would see a panel popping up on the right for generating headlines with or without AI assistance which was the only difference across conditions (see Figure \ref{fig:manual}). 
After finishing generating each news headline, participants were asked to rate how difficult it was to create the headline with the system (see Figure \ref{fig:selection}, \ref{fig:guidance-selection} and \ref{fig:guidance-selection-post-edit}). 
%
Finally, participants completed a \textit{post-task survey} after they finished the task of writing headlines for all 20 articles (see Figure \ref{fig:post-study}).

\subsubsection{Phase II: Human evaluation of headline quality}\hfill

\label{sec:humaneval}

% \subsection{Measures}
%\alison{did we have hypotheses? those should be here as well} \ja{actually our hypotheses are very different from results, do we still need hypotheses?}
% \label{sec:stu1measure}

% Exploring AI-assisted news headline generation, we reported on \textit{headline quality}, \textit{efficiency}, and \textit{user experience}.

%\subsection{Measures for RQ1: Human evaluation of headline quality}
\label{sec:method_performance}
% \alison{the below could be more concise - I can take a pass on it later}
\noindent{\it Participants}
To evaluate the quality of the headlines generated in our study, we recruited a distinct set of 20 evaluators using Upwork.\footnote{We recruited expert annotators on Upwork to attain higher quality ratings.}
% \joel{a few things: 1. in 3.4.1 we specify the backgrounds of the raters, but here we do not.  Why?  It looks inconsistent.  2. not sure what AMT is mentioned here.  Unless we discuss it elsewhere.  I say take it out if it isn't.  Also, if we were to leave it in, the acronym was never explained \alison{removed the bit about AMT}}

%Previous work on human-AI collaborated text generation evaluated generated text with crowdsourcing for a reader perspective such as Amazon Mechanical Turk \cite{kimAbstractiveSummarizationReddit2019}. 
%We recruited expert annotators on Upwork to guarantee high quality ratings.
%
%, meaning it would take 10 annotators to rank all 800 headlines from the user study. 
%For a replication factor of 2, we recruited 20 annotators.

\noindent{\it Procedure}
% \alison{is the interface for this evaluation in the appendix? if not, can you add it and reference it here as well?} \ja{we used excel form for evaluation and I didn't have the raw form on my end}
In the Phase I study, 10 participants wrote headlines for 20 articles across 4 conditions, resulting in 800 headlines for the expert evaluation in Phase II. 
%
Those 800 headlines were evaluated alongside the 20 original news article headlines (\textit{baseline}) and the 20 headlines generated by GPT-3.5 without human intervention (\textit{GPT only}).
%
Achieving a replication factor of 2 required evaluation of 1680 headlines.
%
Therefore, each of the 20 annotators evaluated 80 headlines from the human study (4 human conditions x 20 articles) and 40 headlines from the other groups (\textit{baseline} and \textit{GPT only}). We prepared Excel forms with instructions, news articles, and news headline ranking tables and distributed them to evaluators.
% shown below - for expert evaluation:

%\begin{itemize}
%    \item \textit{Baseline}: original headlines written by professional editors;
%    \item \textit{GPT only}: GPT generated headlines (without any human intervention).
%\end{itemize}

% \alison{the following two sentences need a little clarification}
 
The annotators ranked the quality of the headlines based on the Taste-Attractiveness-Clarity-Truth (TACT) test\footnote{http://www.columbia.edu/itc/journalism/isaacs/client\_edit/\\Headlines.html} from 1 (best) to 6 (worst) as shown below. The annotators were asked to give reasons for their ranking of each headline, and they were able to give the same ranking to two or more headlines for the same article if they were of similar quality.

\begin{itemize}
    \item Taste: Is it in good taste? Is there anything possibly offensive in the headline? Can anything in the headline be taken the wrong way?
    \item Attractiveness: Is it attractive to the reader? Can it be improved so it is more engaging and interesting, without sacrificing accuracy?
    \item Clarity: Does it communicate the key points of the article? Is it clear and simple? Does it use the active voice and active verbs? Are there any odd words or double meanings that could confuse the reader?
    \item Truth: Is it accurate? Are the proper words or terms from the article used in the headline? Is the headline factually correct?
\end{itemize}

% There were 42 headlines associated with each news article.
Each annotator ranked six unique headlines (one from each of the compared groups without duplicates) for each of the 20 articles.  
%
In fact, there were only a few duplicated headlines, meaning the same headlines were generated by GPT-3.5 and selected by different participants (11/840, 1.3\%). Evaluating agreement among evaluators posed a challenge due to the differential ranking of each headline. To quantify this agreement, we applied \textit{Fleiss' kappa} \cite{fleiss1971measuring}, a statistical measure designed to assess the reliability of concurrence among a fixed set of raters classifying items categorically. Specifically, we used this measure on headlines from the \textit{Baseline} and \textit{GPT only} conditions, each of which was ranked by 20 evaluators. The computed average \textit{Fleiss' kappa} for 40 headlines from both the \textit{Baseline} and \textit{GPT only} conditions was 0.027, suggesting a low level of agreement.

%We ensured that annotators were not asked to review duplicate headlines.\footenote{} 
%
%From our pilot of the expert evaluation, the evaluation of 1 news article with 6 headlines took around 3 minutes. 
We paid \$20 to each participant the Phase II evaluation task (estimating 1 hour based on piloting the task).\footnote{In our pilot, evaluating one news article with six headlines took around three minutes.}
%for a 1-hour evaluation of 20 articles (similar scale to the 1-hour user study).

\subsection{Measures}
We report on headline quality, task efficiency, and user experience for the headline generation task.
%
Headline quality is measured using human ratings (Section \ref{sec:humaneval}).
%
For task efficiency, we collect the 1) article reading time (time between starting reading one news article and clicking ``Continue to Write Headline'');
2) headline creation time (time between clicking ``Continue to Write Headline'' and clicking ``Submit Headline''); and 3) overall time (article reading time + headline creation time). For comparing efficiency between conditions, we are most interested in the headline creation time. 

We measured user experience with three subjective measures. 
%
Participants reflected on \textit{Task difficulty} both after each headline (instance-level) and after completing all headlines. %
For instance-level task difficulty, participants answered ``How difficult was it to create this headline for the news article with the system?'' using a slider from 0 (very easy) to 100 (very difficult).
%
For overall difficulty, they specified agreement with ``It was difficult to create headlines for the news articles with the system.'' on Likert scale from 1 (strongly disagree) to 5 (strongly agree) and answered a follow-up ``why do you feel this way?''. 
%
Using measures from prior work, we also collected participants perceived \textit{control}, ``I could influence the final headlines for the news articles''~\cite{raderExplanationsMechanismsSupporting2018a}, and \textit{trust}, ``I trusted that the system would help me create high-quality headlines''~\cite{cramerEffectsTransparencyTrust2008}, with 5-point Likert rating scales (from strongly disagree to strongly agree).
% \begin{itemize}
  %  \item a) participants' self-rating on \textit{task difficulty} after each task with NASA TLX slider from 0 (very easy) to 100 (very difficult) on question "How difficult was it to create this headline for the news article with the system?";
  %  \item b) participants' rating on overall \textit{task difficulty} with a Likert scale rating from 1 (strongly disagree) to 5 (strongly agree) on the statement "It was difficult to create headlines for the news articles with the system." and a follow-up question "Why do you feel this way?";
   % \item c) participants' rating on \textit{control} \& \textit{trust} on the headline generation system with Likert scale ratings from 1 (strongly disagree) to 5 (strongly agree) on two statements "I could influence the final headlines for the news articles" and "I trusted that the system would help me create high-quality headlines" based on previous works \cite{raderExplanationsMechanismsSupporting2018a} and \cite{cramerEffectsTransparencyTrust2008} respectively.
% \end{itemize}

\subsection{Data analysis}
\label{sec:analysis}
%We analyze the quantitative measures (headline quality, efficiency, and task difficulty) using comparing headline quality, we have six groups (four study conditions, AI-only, and the original headlines--baseline).
The quantitative results of headline quality rankings, task efficiency, and average and overall task difficulties, and perceived control and trust ratings were tested by Kruskal-Wallis H test \cite{kruskalUseRanksOneCriterion}, the non-parametric version of one-way Anova test for data with three or more conditions. We then conducted pairwise comparison of headline quality using Mann-Whitney U test \cite{mannTestWhetherOne1947}, the non-parametric version of the Student t-test for two conditions. 
For headline quality, we compared the four conditions (\textit{Manual}, \textit{Selection}, \textit{Guidance + Selection}, and \textit{Guidance + Selection + Post-editing}) against the original headlines (\textit{Baseline}) and automatic method (\textit{GPT only}). For task efficiency and user experience, we compared only within the four human study conditions.
% \alison{we didn't code right?} \ja{no we didn't code}
We also reviewed qualitative results - participants' general comments and comments on task difficulty - and did a case study of evaluators' ranking.

% In the Analysis Of Variance (ANOVA), we assume that the dependent variable is normally distributed and there is approximately equal variance on the scores across groups. However, when using the Kruskal-Wallis Test, we do not have to make any of these assumptions. We are comparing ordinal data and non-normal (long tailed) data so we need to use Kruskal-Wallis.

==> sections/methods-prev-2.tex <==
\section{Evaluating AI-assisted news headline generation}

Our study focused on three research questions (RQs): \textbf{RQ1}: How do different forms of assistance affect quality? Is AI alone good enough or is human input needed for high quality?
\textbf{RQ2}: How do different forms of assistance affect effort (task time and perceived difficulty)? \textbf{RQ3}: How do different forms of assistance affect feelings of ownership (perceived control) and trust? 

To answer those RQs, we explored how three variants of AI-assisted news headline generation affect headline quality (RQ1), effort (RQ2), and sense of ownership and trust (RQ3), compared to fully manual or fully automatic approaches.

\subsection{Task}
We chose to study AI-assisted text generation in the context of news headline generation due in part to the task familiarity---news is an accessible text domain and many already have a sense of what makes a good (or bad) news headline. Further, writing high-quality news headlines requires a balance of creativity and accuracy beyond simple text summarization, yet takes less time and effort than long-form summarization, such as writing paper abstracts or news article summaries.  
Finally, news headlines are easier to evaluate than more open-ended or longer-form content generation tasks.

\subsection{AI-assisted news headline generation types and system variants}

We explored four headline writing variants: writing manually or assisted by AI using one of three common human-AI interaction types identified by prior work \cite{chengMappingDesignSpace2022}:
\textit{guidance} of the LLM headline generation with perspectives (keywords or facets), \textit{selection} from three LLM-generated headlines, and \textit{post-editing} the LLM-generated headline.

As we are interested in understanding the tradeoffs between control and effort in AI-assisted generation tasks, we chose to compound the different interaction types instead of exploring them separately.

Specifically, we developed an AI-assisted news headline generation system with four variants of human-AI interactions:
\begin{itemize}
    \item \textit{Selection}: LLM generates three headlines for each news article (\textit{generate headlines}) and the user chooses the best headline;
    \item \textit{Guidance + Selection}: LLM extracts several potential perspectives (keywords) for each news article (\textit{extract perspectives}), the user chooses one or more perspectives to emphasize in the headline, then LLM generates three headlines for each news article based on the selected perspectives (\textit{generate headlines w/ perspectives}), and, finally, the user chooses the best headline;
    \item \textit{Guidance + Selection + Post-editing}: the same as \textit{Guidance + Selection} but the user is further able to edit the chosen headline (post-editing);
    \item \textit{Manual only}: the participant writes news headline without any assistance.
\end{itemize}

\subsection{System Implementation}
The system was built on the React and Redux front-end frameworks and used Firebase real-time database to store user interaction data. We chose OpenAI's GPT-3.5 \textit{text-davinci-002} model, the state-of-the-art LLM when the study was conducted (July 2022) for the model. The frontend directly called  OpenAI's GPT-3.5 API using prompt programming (see below) to \textit{extract perspectives} (keywords) and \textit{generate headlines}---with and without supplied perspectives---and presents the results to the user (see Figure \ref{fig:interface} as an example). 

To determine the optimal prompts for \textit{extract perspectives}, \textit{generate headlines}, and \textit{generate headlines w/ perspectives} with the GPT-3.5 API, we tested several configurations, and chose the zero-shot learning paradigm (no examples of news headlines included) for broad coverage of news topics. Below are the finalized prompts for corresponding tasks:
\begin{itemize}
    \item \textit{extract perspectives}: "Please identify five keywords and key phrases (nouns) for the following news article.\textbackslash nNews article:\textbackslash n + [news article] + \textbackslash nFive keywords and key phrases (nouns), separated with comma:\textbackslash n"
    \item \textit{generate headlines}: "Please come up with three high-quality (attractive, clear, accurate and inoffensive) headlines for the following news article.\textbackslash nNews article:\textbackslash n\textbackslash n + [news article] + \textbackslash n\textbackslash nThree high-quality headlines:\textbackslash n"
    \item \textit{generate headlines w/ perspectives}: "Please come up with three high-quality (attractive, clear, accurate and inoffensive) headlines for the following news article including keyword(s): [keyword(s) selected by participants].\textbackslash nNews article:\textbackslash n\textbackslash n + [news article] + \textbackslash n\textbackslash nThree high-quality headlines:\textbackslash n"
\end{itemize}
\joel{are all these newline commands supposed to be in the above?  It looks weird.}
GPT-3.5 API takes the above prompts and returns the requested outputs.

To thoroughly test the reliability of LLMs, we utilized a temperature setting of 1, maximizing the variety in the output. Additionally, we set a token count of 400, ensuring an adequate allowance for both input data - comprising prompts and news articles - and output data, which included several keywords or news headlines.

\begin{figure*}
    \centering \includegraphics[width=0.6\textwidth]{figures/Interface.png}
    \caption{AI-assisted news headline generation interface for \textit{guidance + selection + post-editing} condition: (A) news reading panel, (B) perspectives (keywords) selection panel (multiple keywords can be selected), (C) headline selection panel with post-editing capability, and (D) difficulty rating slider. Note: (B), (C) and (D) are hidden from the user until the requisite step is finished (e.g., the user does not see the difficulty rating slider until after finalizing the headline). 
    Interface variants for all study conditions can be found in the Appendix \ref{appendix:a}.}
\label{fig:interface}
\end{figure*}

--todo

\subsection{Study design}
\label{sec:studydesign}
This study consisted of two phases: (1) AI-assisted news headline generation and (2) human evaluation of the generated headlines.
%
The first phase followed a between-subjects experimental design with four conditions, from least human control to maximal human control: (1) \textit{Selection}, (2) \textit{Guidance + Selection}, (3) \textit{Guidance + Selection + Post-editing} and (4) \textit{Manual only}. In the second phase, human evaluators ranked the headlines generated in the first phase and headlines from two baseline conditions.

\subsubsection{Phase I: AI-assisted headline generation}\hfill\\
\newline
\noindent{\it Participants} We recruited 40 participants, 10 per condition on a freelancing platform Upwork\footnote{https://www.upwork.com/} (28 females, 11 males, 1 non-binary) who read news articles with relatively high frequency: a few times a day (29) or a few times a week (11). All of the participants had experience in journalism, editing or writing. Education backgrounds were varied: Bachelor's Degree: 18, Master's Degree: 11, Some High School or High School: 10, Prefer not to say: 1).

\noindent{\it Procedure} The study participants crafted headlines for 20 articles\footnote{The chosen articles ranged from 300 to 1000 words.} (in June 2022) from Yahoo! News\footnote{https://news.yahoo.com/}, the most popular news website in US (Q1 2022)\footnote{https://today.yougov.com/ratings/entertainment/popularity/\\news-websites/all} across four distinct themes: World Politics, COVID-19, Climate Change, and Science, with each topic encompassing five articles. To prevent the possibility of eliciting negative emotional responses or influencing participant behavior, news pertaining to Domestic and US politics was purposefully omitted from the study. The overall study procedure includes a study instruction round, practice round, human study, and a post-task survey. Each participant was randomly assigned to one of the four study conditions and paid \$20 for their 1-hour participation.

Participants first completed the \textit{study instruction}, where they learn how to use the system assigned to them with different types of AI assistance (see screenshots in Appendix \ref{appendix:a} as Figure \ref{fig:inst1} and Figure \ref{fig:inst2}). 
%
Then participants were asked to write headlines for 2 practice articles (\textit{practice round}) before moving on to the \textit{human study}, which involved writing headlines for 20 task articles.
For each article, participants first read the article and then click “Continue to Write Headline" after they finish reading.

Then they would see a panel popping up on the right for generating headlines with or without AI assistance which was the only difference across conditions (see Figure \ref{fig:manual}). 
After finishing generating each news headline, participants were asked to rate how difficult it was to create the headline with the system (see Figure \ref{fig:selection}, \ref{fig:guidance-selection} and \ref{fig:guidance-selection-post-edit}). 
%
Finally, participants completed a \textit{post-task survey} after they finished the task of writing headlines for all 20 articles (see Figure \ref{fig:post-study}).

\subsubsection{Phase II: Human evaluation of headline quality}\hfill

\label{sec:humaneval}

\label{sec:method_performance}
\noindent{\it Participants}
To evaluate the quality of the headlines generated in our study, we recruited a distinct set of 20 evaluators using Upwork.\footnote{We recruited expert annotators on Upwork to attain higher quality ratings.}

\noindent{\it Procedure}
In the Phase I study, 10 participants wrote headlines for 20 articles across 4 conditions, resulting in 800 headlines for the expert evaluation in Phase II. 

Those 800 headlines were evaluated alongside the 20 original news article headlines (\textit{baseline}) and the 20 headlines generated by GPT-3.5 without human intervention (\textit{GPT only}).

Achieving a replication factor of 2 required evaluation of 1680 headlines.

Therefore, each of the 20 annotators evaluated 80 headlines from the human study (4 human conditions x 20 articles) and 40 headlines from the other groups (\textit{baseline} and \textit{GPT only}). We prepared Excel forms with instructions, news articles, and news headline ranking tables and distributed them to evaluators.

The annotators ranked the quality of the headlines based on the Taste-Attractiveness-Clarity-Truth (TACT) test\footnote{http://www.columbia.edu/itc/journalism/isaacs/client\_edit/\\Headlines.html} from 1 (best) to 6 (worst) as shown below. The annotators were asked to give reasons for their ranking of each headline, and they were able to give the same ranking to two or more headlines for the same article if they were of similar quality.

\begin{itemize}
    \item Taste: Is it in good taste? Is there anything possibly offensive in the headline? Can anything in the headline be taken the wrong way?
    \item Attractiveness: Is it attractive to the reader? Can it be improved so it is more engaging and interesting, without sacrificing accuracy?
    \item Clarity: Does it communicate the key points of the article? Is it clear and simple? Does it use the active voice and active verbs? Are there any odd words or double meanings that could confuse the reader?
    \item Truth: Is it accurate? Are the proper words or terms from the article used in the headline? Is the headline factually correct?
\end{itemize}

Each annotator ranked six unique headlines (one from each of the compared groups without duplicates) for each of the 20 articles.  

In fact, there were only a few duplicated headlines, meaning the same headlines were generated by GPT-3.5 and selected by different participants (11/840, 1.3\%). Evaluating agreement among evaluators posed a challenge due to the differential ranking of each headline. To quantify this agreement, we applied \textit{Fleiss' kappa} \cite{fleiss1971measuring}, a statistical measure designed to assess the reliability of concurrence among a fixed set of raters classifying items categorically. Specifically, we used this measure on headlines from the \textit{Baseline} and \textit{GPT only} conditions, each of which was ranked by 20 evaluators. The computed average \textit{Fleiss' kappa} for 40 headlines from both the \textit{Baseline} and \textit{GPT only} conditions was 0.027, suggesting a low level of agreement.

We paid \$20 to each participant the Phase II evaluation task (estimating 1 hour based on piloting the task).\footnote{In our pilot, evaluating one news article with six headlines took around three minutes.}

\subsection{Measures}
We report on headline quality, task efficiency, and user experience for the headline generation task.
%
Headline quality is measured using human ratings (Section \ref{sec:humaneval}).

For task efficiency, we collect the 1) article reading time (time between starting reading one news article and clicking ``Continue to Write Headline'');
2) headline creation time (time between clicking ``Continue to Write Headline'' and clicking ``Submit Headline''); and 3) overall time (article reading time + headline creation time). For comparing efficiency between conditions, we are most interested in the headline creation time. 

We measured user experience with three subjective measures. 

Participants reflected on \textit{Task difficulty} both after each headline (instance-level) and after completing all headlines. %
For instance-level task difficulty, participants answered ``How difficult was it to create this headline for the news article with the system?'' using a slider from 0 (very easy) to 100 (very difficult).

For overall difficulty, they specified agreement with ``It was difficult to create headlines for the news articles with the system.'' on Likert scale from 1 (strongly disagree) to 5 (strongly agree) and answered a follow-up ``why do you feel this way?''. 

Using measures from prior work, we also collected participants perceived \textit{control}, ``I could influence the final headlines for the news articles''~\cite{raderExplanationsMechanismsSupporting2018a}, and \textit{trust}, ``I trusted that the system would help me create high-quality headlines''~\cite{cramerEffectsTransparencyTrust2008}, with 5-point Likert rating scales (from strongly disagree to strongly agree).

\subsection{Data analysis}
\label{sec:analysis}
The quantitative results of headline quality rankings, task efficiency, and average and overall task difficulties, and perceived control and trust ratings were tested by Kruskal-Wallis H test \cite{kruskalUseRanksOneCriterion}, the non-parametric version of one-way Anova test for data with three or more conditions. We then conducted pairwise comparison of headline quality using Mann-Whitney U test \cite{mannTestWhetherOne1947}, the non-parametric version of the Student t-test for two conditions. 
For headline quality, we compared the four conditions (\textit{Manual}, \textit{Selection}, \textit{Guidance + Selection}, and \textit{Guidance + Selection + Post-editing}) against the original headlines (\textit{Baseline}) and automatic method (\textit{GPT only}). For task efficiency and user experience, we compared only within the four human study conditions.

We also reviewed qualitative results - participants' general comments and comments on task difficulty - and did a case study of evaluators' ranking.

==> sections/relatedWork-prev-1.tex <==
\section{Related Work}

Our research was built upon previous work on applications of Large Language Models, human-AI interactions for text summarization and news headline generation.

% \alison{also, throughout, make it clear how our work compares/builds on/differentiates from related work (i.e., why should the reader know about this related work? how is it relevant to our paper?}

\subsection{Applications of Large Language Models}
% \alison{this can introduce LLMs and some standalone apps briefly, but should really focus on human-ai co-creation}
% Definition of Large Language Models

Large Language Models (LLMs) such as Generative Pre-trained Transformer (GPT) \cite{brownLanguageModelsAre2020} are attracting attention from researchers and practitioners with their power in generating human-like continuations based on a prompt (a string of text) \cite{bommasaniOpportunitiesRisksFoundation2021, jakeschCoWritingOpinionatedLanguage, leeCoAuthorDesigningHumanAI2022a} and widely used in various text generation tasks from  summarization \cite{dangTextGenerationSupporting2022} to storytelling \cite{yuanWordcraftStoryWriting2022a, singhWhereHideStolen2022}. Their unprecedented generality is from their capability of zero-shot and few-shot learning that task-specific training data is not required.
% especially in processing small-scale text data and prompts and generating text outputs (up to ~3000 words in total).
% \joel{we should be a bit careful as some people might claim that few-shot is a type of fine-tuning.  These models work well when there is some task specific data for sure.}  \cite{brownLanguageModelsAre2020}. 
\alison{are all the following examples cases where humans interact with LLMs for some task? or just use their outputs for some other task? or a mix?}
Proof-of-concept usages of LLMs included text summaries for writers \cite{dangTextGenerationSupporting2022}, medical dialogue summarization \cite{chintaguntaMedicallyAwareGPT32021}, story creation \cite{yuanWordcraftStoryWriting2022a, singhWhereHideStolen2022}, metaphor generation \cite{chakrabartyMERMAIDMetaphorGeneration2021}, movie review \cite{bhatInteractingNextphraseSuggestions2023}, scientific content generation \cite{geroSparksInspirationScience2022}, learning content creation \cite{macneilAutomaticallyGeneratingCS2022}, code explanation \cite{macneilExperiencesUsingCode2022, macneilGeneratingDiverseCode2022}. 
% \ja{Todo: adding details of how human interact with those applications: autocomplete, suggestion}
% The high quality of LLM-generated text was  exemplified by that ChatGPT\footnote{https://chat.openai.com/chat}, a LLM-powered chatbot, was even listed as authors of academic papers \cite{stokel-walkerCHATGPTLISTEDAUTHOR, generativepre-trainedtransformerRapamycinContextPascal2022, transformerCanGPT3Write}.\joel{this previous sentence doesn't make sense.  Is the point that ChatGPT is so good that it is being used an author on papers?  We should be careful here because at least one AI conference said it couldn't be used for writing papers.  I would just find better examples or not include it.  }
% Outside the research community, LLMs have been applied for content generation\footnote{https://www.regie.ai/, https://www.copy.ai/, https://writer.com/}, writing assistant\footnote{https://www.compose.ai/, https://www.notion.so/product/ai} and code generation\footnote{https://github.com/features/copilot}.
% \joel{the footnotes do not back up the claim that there are widely used.  Either you have a citation for it or it should be taken out.}

% \joel{section 2.1 doesn't match the section heading.  The content of the section seems to be a quick list of areas where LLMs perform well.  However there is nothing about co-creation specifically, which is the section header.  So the section should either be about LLMs or include more content about how these models have been used in co-creation environments}

% creative writing \cite{clarkCreativeWritingMachine2018, yuanWordcraftStoryWriting2022a, roemmeleWritingStoriesHelp2016, singhWhereHideStolen2022, berkovskyHowNovelistsUse2018, freiknechtProceduralGenerationInteractive2020, geroMetaphoriaAlgorithmicCompanion2019}
%essays \cite{dangTextGenerationSupporting2022} 

%What we know about GPT-3 to generate quality results
%Provide clear prompt programming of tasks
%Break down logical steps
%Provide guidance for each step and context information

\subsection{Human-AI interactions for text summarization}
% \alison{this jumps too quickly into the three types that we happen to use - would be better to first talk about how prior work (regina) provides a taxonomy of common types (list them) and say that we choose to study these three in particular - also include any other prior work that surveys/summarizes different types aside from Regina work..}
% \alison{also there are a ton of cites here.. i think just taken from REginas? maybe we choose just 1-2 representative cites for each type instead of listing all?}

Cheng et al. \cite{chengMappingDesignSpace2022} reviewed 70 papers involving AI-assisted text generation systems and synthesized a taxonomy of common types of of human-AI interactions for text generation: 1) \textit{guiding model output}, 2) \textit{selecting or rating model output}, 3) \textit{post-editing}, 4) \textit{interactive editing} and 5) \textit{writing with model assistance}. Since the later two types are often used for complex and open-ended text generation tasks \cite{chengMappingDesignSpace2022}, we focus on the first three types in this paper which are more suitable for the concrete text summarization tasks. Importantly, these interactions vary in the level of control they provide over the final output, as well as the level of effort they require of the human.

%
When \textit{Guiding model output} humans control or \textit{guide} the automatic text generation process. For example, humans can specify important parts of some input text which should be included in the output \cite{pouliquenTaptaUserdrivenTranslation, gehrmannVisualInteractionDeep2019}, provide semantic prompts (e.g., keywords, facets, or written prompts) for the generation \cite{ghazvininejadHafezInteractivePoetry2017, clarkCreativeWritingMachine2018, osoneBunChoAISupported2021, changChangingMindTransformers2021, strobeltGenNIHumanAICollaboration2022}, or  provide style parameters (e.g., sentiment, length of text) desired in the output \cite{ghazvininejadHafezInteractivePoetry2017, freiknechtProceduralGenerationInteractive2020}.
%
For our study, humans guide the headline generation by specifying keyword (or perspective) prompts that should be included in the generated headlines.

Alternatively, \textit{selecting or rating model output} happens after the text generation process has occurred. Here, humans choose from multiple model outputs \cite{pouliquenTaptaUserdrivenTranslation, kreutzerReliabilityLearnabilityHuman2018, rosaTHEaiTREArtificialIntelligence2020, stiennonLearningSummarizeHuman} or give a rating over all outputs \cite{nguyenReinforcementLearningBandit2017, lamReinforcementLearningApproach2018, lamInteractivePredictiveNeuralMachine2019, bohnHoneYouRead2021, wuRecursivelySummarizingBooks2021}.
%
In our study, humans choose from three generated headlines.
%\textit{Guiding model output} enables moderate level of human control on AI, and is associated with high level of efficiency and human trust on AI \cite{chengMappingDesignSpace2022}. 


%The \textit{selecting or rating model output} interaction is mainly based on multiple choices \cite{pouliquenTaptaUserdrivenTranslation, kreutzerReliabilityLearnabilityHuman2018, rosaTHEaiTREArtificialIntelligence2020, stiennonLearningSummarizeHuman} and rating \cite{nguyenReinforcementLearningBandit2017, lamReinforcementLearningApproach2018, lamInteractivePredictiveNeuralMachine2019, bohnHoneYouRead2021, wuRecursivelySummarizingBooks2021}.

Finally, humans can edit generated text (\textit{post-editing}). Typically this occurs in a free-form text box \cite{laiExplorationPostEditingEffectiveness2022, denkowskiChallengesPredictingMachine, yamaguchiEvaluationRewritingService2013, turchiDatadrivenAnnotationBinary2014, chuTranSearchMultilingualSearch2017, huangAISONGCONTEST2020, moramarcoBabylonHealthLondon}, but could also be complemented with suggestions for edits (e.g., substitution dropdowns) \cite{liuComputerAssistedWriting2011, shiAgentMetaphorMachine2013, weiszPerfectionNotRequired2021, passaliHumanCenteredSummarizationCase}, %scaffold for context (e.g., embedded dictionary) \cite{sugiyamaAssistingUsersCrosscultural2011}, 
or other productivity supports (e.g., auto-correction) \cite{lagardaTranslatingIndomainCorpus2015, perisOnlineLearningEffort2019, wangComputerAssistedTranslation2020, zhaoBalancingQualityHuman2020, weiszPerfectionNotRequired2021}. 
%
We study inline post-editing of the selected headline without any additional support.

%\textit{Selecting or rating model output} focuses on a high level of efficiency while sacrificing the level of control and trust on AI as humans can only judge but not change AI-generated contents. 

%\textit{post-editing} is associated with a high level of control on AI by enabling human to directly edit AI-generated outputs, and a moderate level of efficiency and trust on AI. Those interactions with different focuses and participants’ perceptions of the level of control on AI, trust on AI, and efficiency constituted the conditions of human-AI interaction in this paper.

\subsection{News headline generation and evaluation}

News headline generation was conventionally considered as a paradigm of text summarization tasks and has been widely studied \cite{alfonsecaHEADYNewsHeadline, tanNeuralSentenceSummarization2017, goyalNewsSummarizationEvaluation2022}. Its fully automated solutions have evolved from heuristics approaches, such as  parse-and-trim  \cite{dorrHedgeTrimmerParseandtrim2003}, to more advanced machine learning algorithms, such as recurrent neural networks \cite{lopyrevGeneratingNewsHeadlines2015}, Universal Transformer \cite{gavrilovSelfAttentiveModelHeadline2019}, reinforcement learning \cite{songAttractiveFaithfulPopularityReinforced2020, xuClickbaitSensationalHeadline2019}, 
% deep learning \cite{passaliHumanCenteredSummarizationCase},\joel{it's weird to have deep learning as one of the list items when three of the other list items are deep learning as well.  } 
large-scale generation models trained with a distant supervision approach \cite{guGeneratingRepresentativeHeadlines2020}. Those studies of news headline generation focused on fully automated algorithms while human aspects in those studies are primarily for evaluation instead of creation. The evaluation of generated news headlines include case study \cite{guGeneratingRepresentativeHeadlines2020, muraoCaseStudyNeural2019}, human rating 
\cite{dorrHedgeTrimmerParseandtrim2003, songAttractiveFaithfulPopularityReinforced2020} and annotating \cite{xuClickbaitSensationalHeadline2019}. Besides being a testbed for text summarization, news headline generation also has a real-world impact on the journalism industry, as journalists may benefit from news headline generation algorithms to save both time and effort. 
% As of 2023, over 3,500 newspaper publishing businesses are in the US\footnote{https://www.ibisworld.com/industry-statistics/number-of-businesses/newspaper-publishing-united-states}.\joel{this prior sentence doesn't explain why headline generation has a real world impact}
% Similar to other types of online content, many news headlines are created and selected through algorithms such as the multi-armed bandit approach \cite{maoBatchedMultiArmedBandit2018}, which makes it time-consuming and challenging for journalists to come up with substantial high-quality headlines.\joel{I am not sure that entailment works.  The 2018 paper cited shows an approach to test different headlines in the real world andthen pick the must delectable one.  I am not sure it delves into the time required to write the headlines.} Therefore journalists may benefit from news headline generation algorithms to save both time and effort.

% For example, the creation of tweetorials - short and technical explanations written on Twitter for a general audience - were used for studying human-AI interaction in science writing \cite{geroSparksInspirationScience2022}..

%  Digital creativity support for journalists \cite{maidenMakingNewsDigital2018}

%  News studied in CHI \cite{lapidesNewsFeedWhat2015}

==> sections/relatedWork-prev-2.tex <==
\section{Related Work}

Our research was built upon previous work on applications of Large Language Models, human-AI interactions for text summarization and news headline generation.

\subsection{Applications of Large Language Models}

Large Language Models (LLMs) such as Generative Pre-trained Transformer (GPT) \cite{brownLanguageModelsAre2020} are attracting attention from researchers and practitioners with their power in generating human-like continuations based on a prompt (a string of text) \cite{bommasaniOpportunitiesRisksFoundation2021, jakeschCoWritingOpinionatedLanguage, leeCoAuthorDesigningHumanAI2022a} and widely used in various text generation tasks from  summarization \cite{dangTextGenerationSupporting2022} to storytelling \cite{yuanWordcraftStoryWriting2022a, singhWhereHideStolen2022}. Their unprecedented generality is from their capability of zero-shot and few-shot learning that task-specific training data is not required.
 
Proof-of-concept usages of LLMs included text summaries for writers \cite{dangTextGenerationSupporting2022}, medical dialogue summarization \cite{chintaguntaMedicallyAwareGPT32021}, story creation \cite{yuanWordcraftStoryWriting2022a, singhWhereHideStolen2022}, metaphor generation \cite{chakrabartyMERMAIDMetaphorGeneration2021}, movie review \cite{bhatInteractingNextphraseSuggestions2023}, scientific content generation \cite{geroSparksInspirationScience2022}, learning content creation \cite{macneilAutomaticallyGeneratingCS2022}, code explanation \cite{macneilExperiencesUsingCode2022, macneilGeneratingDiverseCode2022}. 

\subsection{Human-AI interactions for text summarization}

Cheng et al. \cite{chengMappingDesignSpace2022} reviewed 70 papers involving AI-assisted text generation systems and synthesized a taxonomy of common types of of human-AI interactions for text generation: 1) \textit{guiding model output}, 2) \textit{selecting or rating model output}, 3) \textit{post-editing}, 4) \textit{interactive editing} and 5) \textit{writing with model assistance}. Since the later two types are often used for complex and open-ended text generation tasks \cite{chengMappingDesignSpace2022}, we focus on the first three types in this paper which are more suitable for the concrete text summarization tasks. Importantly, these interactions vary in the level of control they provide over the final output, as well as the level of effort they require of the human.

When \textit{Guiding model output} humans control or \textit{guide} the automatic text generation process. For example, humans can specify important parts of some input text which should be included in the output \cite{pouliquenTaptaUserdrivenTranslation, gehrmannVisualInteractionDeep2019}, provide semantic prompts (e.g., keywords, facets, or written prompts) for the generation \cite{ghazvininejadHafezInteractivePoetry2017, clarkCreativeWritingMachine2018, osoneBunChoAISupported2021, changChangingMindTransformers2021, strobeltGenNIHumanAICollaboration2022}, or  provide style parameters (e.g., sentiment, length of text) desired in the output \cite{ghazvininejadHafezInteractivePoetry2017, freiknechtProceduralGenerationInteractive2020}.
For our study, humans guided the headline generation by specifying keyword (or perspective) prompts that should be included in the generated headlines.

Alternatively, \textit{selecting or rating model output} happens after the text generation process has occurred. Here, humans choose from multiple model outputs \cite{pouliquenTaptaUserdrivenTranslation, kreutzerReliabilityLearnabilityHuman2018, rosaTHEaiTREArtificialIntelligence2020, stiennonLearningSummarizeHuman} or give a rating over all outputs \cite{nguyenReinforcementLearningBandit2017, lamReinforcementLearningApproach2018, lamInteractivePredictiveNeuralMachine2019, bohnHoneYouRead2021, wuRecursivelySummarizingBooks2021}.
In our study, humans could choose from three generated headlines.

Finally, humans can edit generated text (\textit{post-editing}). Typically this occurs in a free-form text box \cite{laiExplorationPostEditingEffectiveness2022, denkowskiChallengesPredictingMachine, yamaguchiEvaluationRewritingService2013, turchiDatadrivenAnnotationBinary2014, chuTranSearchMultilingualSearch2017, huangAISONGCONTEST2020, moramarcoBabylonHealthLondon}, but could also be complemented with suggestions for edits (e.g., substitution dropdowns) \cite{liuComputerAssistedWriting2011, shiAgentMetaphorMachine2013, weiszPerfectionNotRequired2021, passaliHumanCenteredSummarizationCase},
or other productivity supports (e.g., auto-correction) \cite{lagardaTranslatingIndomainCorpus2015, perisOnlineLearningEffort2019, wangComputerAssistedTranslation2020, zhaoBalancingQualityHuman2020, weiszPerfectionNotRequired2021}. 
We studied inline post-editing of the selected headline without any additional support.

\subsection{News headline generation and evaluation}

News headline generation was conventionally considered as a paradigm of text summarization tasks and has been widely studied \cite{alfonsecaHEADYNewsHeadline, tanNeuralSentenceSummarization2017, goyalNewsSummarizationEvaluation2022}. Its fully automated solutions have evolved from heuristics approaches, such as  parse-and-trim  \cite{dorrHedgeTrimmerParseandtrim2003}, to more advanced machine learning algorithms, such as recurrent neural networks \cite{lopyrevGeneratingNewsHeadlines2015}, Universal Transformer \cite{gavrilovSelfAttentiveModelHeadline2019}, reinforcement learning \cite{songAttractiveFaithfulPopularityReinforced2020, xuClickbaitSensationalHeadline2019}, large-scale generation models trained with a distant supervision approach \cite{guGeneratingRepresentativeHeadlines2020}. Those studies of news headline generation focused on fully automated algorithms while human aspects in those studies are primarily for evaluation instead of creation. The evaluation of generated news headlines include case study \cite{guGeneratingRepresentativeHeadlines2020, muraoCaseStudyNeural2019}, human rating 
\cite{dorrHedgeTrimmerParseandtrim2003, songAttractiveFaithfulPopularityReinforced2020} and annotating \cite{xuClickbaitSensationalHeadline2019}. Besides being a testbed for text summarization, news headline generation also has a real-world impact on the journalism industry, as journalists may benefit from news headline generation algorithms to save both time and effort.

==> sections/results-prev-1.tex <==
\section{Results}

% \subsection{Results of editors' headline generation efficiency and experience}

We report on the results of headline quality (RQ1), task effort---efficiency and perceived difficulty (RQ2), and control and trust (RQ3) for the different AI-assisted text generation conditions.
%


%1) task efficiency and experience (from Section \ref{sec:efficiency} to Section \ref{sec:comment}), and 2) task performance (Section \ref{sec:quality} and Section \ref{sec:casestudy}).


% HEADLINE QUALITY
\subsection{GPT-3.5 only produced the best headlines while manual and selection-only methods produced the worst}
%\subsubsection{GPT only produced the best headlines while manual and selection-only methods produced the worst}
\label{sec:quality}

We compared the quality of the generated headlines between six groups: the four AI-assisted conditions, manual, and automatic methods based on human rankings (see Section~\ref{sec:humaneval})
%and corresponding significance tests (see Section~\ref{sec:analysis}).
%
and collected 2390 rankings (1st to 6th)\footnote{10 codes were missed due to annotator error} from 20 annotators (Table~\ref{tab:eval}). 
%

 
%with writing or editing experience and having not participated the human study. 
%
%The counts of rankings are reported in . %
The six generated headline groups significantly differed in quality rankings (Kruskal-Wallis H tests, $H-value=50.8, p-value<0.01$). 
%
Further pairwise comparison of the groups (Table \ref{tab:pairwise_compare}) provides insight into the differences: 
Participants in the \textit{Manual} condition wrote the worst headlines, and \textit{GPT only} produced the best headlines (aside from the \textit{Baseline}).
%
For the AI-assisted conditions, adding human guidance through providing perspectives (keywords)---(\textit{Guidance + Selection} or \textit{Guidance + Selection + Post-editing})---yielded better headlines than \textit{Selection} alone. 
%
Post-editing did not impact headline quality: there was no significant difference in ranking between the headlines generated in the \textit{Guidance + Selection} and \textit{Guidance + Selection + Post-editing} conditions.

To further compare the groups, we look at the count of ``top'' (ranked 1st) and ``bottom'' (ranked 6th) rankings (Table~\ref{tab:eval}).
%
We correctly anticipated the original headlines for the news articles (\textit{Baseline}) would be the highest quality, receiving the most ``top'' rankings (87) and fewest ``bottom'' rankings (38). 
%
\textit{GPT only}, had fewer ``top'' rankings than \textit{Baseline} (70) but a similar number of ``bottom'' rankings (37). 
%
\textit{Manual} and \textit{Selection} had the fewest ``top'' rankings (56), while \textit{Manual} also had the most bottom rankings (98).
%\textit{Guidance + Selection} and \textit{Guidance + Selection + Post-editing}. 
%
%\textit{Baseline} and \textit{GPT only} also had the least ``bottom'' ranking headlines while \textit{Manual only} had the most.
%
%It was as expected that \textit{Baseline} - the original headlines from news website as the golden standard - had the best quality.
%
%While \textit{GPT only} did not generate as many ``top'' headlines as \textit{Baseline}, it was comparable to \textit{Baseline} and similar or better than \textit{Manual} and the AI-assisted conditions (\textit{Selection}), indicating that GPT alone is promising for generating high quality news headlines.
In Appendix A, Table \ref{tab:casestudy} presents the rankings assigned by one annotator to six headlines, each derived from a different condition, for a single article. Accompanying comments elucidate the rationale behind their ratings—in this case, favoring the succinct headline generated by GPT-3.5 and critiquing the mistake that marred the manually written headline.

To summarize, an approximate comparison of quality ranking among the studied conditions is: \textit{Baseline} $\sim$ \textit{GPT only} > \textit{Guidance + Selection} $\sim$ \textit{Guidance + Selection + Post-editing} > \textit{Selection} $\sim$ \textit{Manual only}.

\begin{table*}[]
\centering
\begin{tabular}{llll}
\hline
\textbf{Condition 1 > Condition 2} & \textbf{U-value} & \textbf{p-value} \\ \hline
\textit{Baseline} > \textit{Manual only} & 61766.0 & <0.01\\
\textit{Baseline} > \textit{Selection} & 63550.0 & <0.01\\
\textit{Baseline} > \textit{Guidance + Selection} & 72364.5 & 0.028\\
\textit{Baseline} > \textit{Guidance + Selection + Post-editing} & 72688.5 & 0.048\\
\textit{GPT only} > \textit{Manual only} & 63168.5 & <0.01\\
\textit{GPT only} > \textit{Selection} & 64751.5 & <0.01\\
\textit{Guidance + Selection} > \textit{Manual only} & 89877.5 & <0.01\\
\textit{Guidance + Selection} > \textit{Selection} & 88536.5 & <0.01\\
\textit{Guidance + Selection + Post-editing} > \textit{Manual only} & 89972.5 & <0.01\\
\textit{Guidance + Selection + Post-editing} > \textit{Selection} & 88734.0 & <0.01\\ \hline
\end{tabular}
\caption{Pairwise comparison of headline quality rankings with significant difference (p<0.05, Mann-Whitney U).}
\label{tab:pairwise_compare}
\end{table*}


%\subsubsection{Case study on headline evaluation}
%\label{sec:casestudy}
%\alison{after reviewing this again, i think its too much detail but I do like the sample of what headlines look like and how someone ranks.. I'm gonna fold it into the above section}
% \alison{I like this detail! it might flow better if it came first before you give all the quality results}

%To better understand how annotators rated the headlines, we conducted a case study for one of the evaluation tasks, looking at six generated headlines, the corresponding rankings, and the annotators' comments (see Table \ref{tab:casestudy}). 
% \alison{what do you mean about the keywords for the news articles for evaluators - did we give them those keywords to look for? or your assessment is that those keywords were important?}
%From the evaluator's comments, we could see the keywords extracted by the evaluator for the news articles were "Army National Guard", "Covid" and "vaccine deadline" (we did not provide a list of keywords to evaluators), and getting those keywords wrong, missing those keywords, ordering those keywords inappropriately or combining those keywords verbosely would lead to a low ranking. The headline produced by \textit{GPT only}, "Army National Guard Faces Recruiting Crisis Amid Covid Vaccine Deadline", included all those keywords in a succinct way and got the top ranking. \textit{Baseline} "Deadline passes and 1 in 10 Army National Guard soldiers still unvaccinated for Covid. Will they be expelled?" included all the necessary information but not concise enough, which was common for \textit{Baseline}. \textit{Manual only} messed up the name of Army National Guard resulted in the lowest ranking, which reflected the possibility of human errors.

%\subsection{RQ2: Effort (efficiency and perceived difficulty)}
\label{sec:efficiency}
\subsection{AI-assisted methods without post-editing were fastest compared to more manual methods}
%\joel{we need to make how we discuss results more consistent.  In 4.1 there is no nice summation in the beginning, one has to wait until the end.}
% \alison{this heading still needs work.. in a gist: more manual methods are slower than more automated methods - we should think about how we want to frame the conditions.. more level of human oversight? human control? human input?}

%Since each participant was paid for one hour to finish the task, the total time they spent was similar (shown in Table \ref{tab:time}). 
We compare headline generation efficiency using \textit{headline creation time}, i.e., the time to generate the news headline, apart from the time to read the news article--\textit{reading time} (Table \ref{tab:time}).
%To observe the difference of task efficiency, we split the time spent on an individual news headline generation task into two parts: \textit{reading time} - the time spent on reading the news article, and \textit{creating time} - the time spent on generating the news headline.

\begin{figure}
    \centering \includegraphics[width=0.5\textwidth]{figures/Creating.png}
    \caption{News headline creation time across four human conditions (standard deviation as error bars): \textit{Selection} and \textit{Guidance + Selection} are faster than the other two conditions which required more human editing (\textit{Manual} and \textit{Guidance + Selection + Post-editing}).}
\label{fig:creating_time}
\end{figure}

As expected, there was no significant difference in \textit{reading time}.\footnote{While similar average reading time across conditions does not necessarily mean similar engagement and task ability for workers in those conditions, it is a promising indicator.}
%
The condition did have an impact on \textit{headline creation time}: the \textit{Selection} and \textit{Guidance + Selection} were significantly faster ($H-value=13.0, p-value=0.005$) than the other conditions which involved manual editing (\textit{Manual} and \textit{Guidance + Selection + Post-editing} (see Figure \ref{fig:creating_time}).

% \subsection{User experience}
%\alison{these measures are all user experience but they tell us much different things (or would have told us different things if they'd been different..), task difficulty is the most important one - another way of describing this study is, we want to know which interaction makes the task easiest (fastest & lowest perceived difficulty) while still achieving high quality output. control and trust are kind of secondary measures, in which interactions do humans feel they have good control and can trust? let's describe the above better in the intro, method, and results}
\subsection{Condition did not impact task difficulty}
\label{sec:difficulty}

% As described in Section \ref{sec:stu1measure}
Overall, the participants did not consider the task to be difficult (average instance-level and overall task difficulties are reported in Table \ref{tab:diff}). 
%
While \textit{Guidance + Selection} had the lowest average instance-level difficulty (M=19.7, SD=24.30) and \textit{Manual} had the highest (M=30.9, SD=17.1), these differences were not significant.
%
This is surprising as manual methods require more human effort (and time) than writing with assistance. We discuss possible reasons for this finding in the Discussion.
%: 1) the mean of average task difficulty was close to 30 for \textit{Manual only}, 2) the means of average task difficulty were less 30 for all AI-assisted conditions, 3) means between 1.7 and 1.9 for the overall task difficulty rating. 
%The results were tested by Kruskal-Wallis H test and there was no significant difference among all four conditions for both average and overall difficulty ratings.

%\alison{Jason - did you do an analysis task difficulty per instance (or did you take average and then compare)? - i wonder if the per instance comparison would have found some differences, because the average doesn't really tell us as much -- its no different than the 'overall' rating at the end.. wondering what Isabel thinks..?} \ja{I took average and then compare because we discussed that each news article might not be representative enough}

\subsection{Qualitative feedback on AI-assisted headline generation}
\label{sec:comment}
% \alison{did you do a full coding of the feedback?} \ja{I went through all the comments and cherry-picked some, but not systematic coding}
%\alison{we probably don't have time..., but would be best to focus on the follow up to task difficulty here (hopefully identifying some nuance between conditions since our scoring didn't..) and then a separate section on the general comments (best if those could align with discussion points)}
After the task, participants provided open-ended responses as a follow-up to their perceived task difficulty and supplied ``any other comments you want to tell us''.
These responses shed light on perceived benefits of AI assistants, for example to aid brainstorming: 

\begin{quote}
"Overall, I'd say this system could definitely be helpful as long as the keyword list lines up with the main keywords in the article. Additionally, it would always be a helpful brainstorming tool for headlines." (P40, \textit{Guidance + Selection + Post-editing}:)
\end{quote}
% (Comment on task difficulty: Some of the headlines were easy to create, and others were difficult. For the ones that were difficult, my biggest problem was choosing keywords that were actually the blatant keywords that I wanted to use. And sometimes the system came up with headlines that weren't related to the keywords I asked for. )

Some participants suggested specific considerations for future AI-assisted systems:
%including coverage of main points in AI-generated headlines (P23), high efficiency but low creativity and reasoning (P39), and guidance on AI model and selection of AI outputs as a non-linear process and more iterations and human-AI interactions needed (P28):

\begin{quote}
    \textbf{Coverage of main points in AI-generated headlines:} "Some of the main points were left out of certain headlines, but otherwise, this proves to be a useful tool for journalists. The main points were combined into an easy-to-use database for selection." (P23, \textit{Guidance + Selection})
\end{quote}
\begin{quote}
    \textbf{High efficiency but low creativity and reasoning:} "I could see how this would be beneficial in situations where time is limited, but it does not replace the creativity and reasoning a human has. Some seemed spot on and others seemed chaotic. But with a few tweaks, it was easy to create a headline. Some of the keywords suggested seemed totally unnecessary. The keywords were the weakest part of the system in my opinion." (P39, \textit{Guidance + Selection + Post-editing})
\end{quote}
\begin{quote}
 \textbf{Guidance on AI model and selection of AI outputs as a non-linear process:} "I do wish I could have gone back to choose different perspectives and see alternate variations than just the 3 original headlines. If those first 3 options don't really cover the central theme of the article, it would be nice to go back and choose alternate perspectives to see if it populates a more precise headline. Overall though, this is a great tool to save time and many headaches.
I really enjoyed this experience and would love to participate again in future exercises." (P28, \textit{Guidance + Selection})
\end{quote}

%\subsection{RQ3: Perceived control and trust}
\subsection{Participants felt similar influence over the final outputs and system trust in all conditions}
\label{sec:results_control}
%\alison{its too late to mod now and I'm sorry for not getting to review this bit sooner, but control is a big piece of what we wanted to study, yet this section is really light.. I know we didn't find any sig difference but it would be good to look at open ended responses and see if anyone talked about influence (particularly in the selection condition where they didn't have much) - something to keep in mind if we do a revision!}
% \subsection{RQ3: All conditions had similar level of control \& trust on the headline generation system}
% \alison{In the past i've used ANOVA to compare Likert data and then do pairwise if theres any significant diff in the group.. how does ANOVA compare to kruskal wallis H?} \ja{The ANOVA (and t-test) is explicitly a test of equality of means of values. The Kruskal-Wallis (and Mann-Whitney) can be seen technically as a comparison of the mean ranks. 

% \alison{it is a little disconcerting that manual didn't do higher for control, right? it seems strange for anyone to give below a 5} \ja{Yes it might be due to the intrinsic headline generation difficulty}

% In the post-study survey, we measured participants' control and trust on the system (with or without AI assistance) with 5-point Likert scale ratings (from 1: strongly disagree to 5: strongly agree) on those two statements: "I could influence the final headlines for the news articles." and "I trusted that the system would help me create high-quality headlines."
Similar to task difficulty, the condition did not impact perceived control or trust (Table \ref{tab:post-survey}).
%Both medians of Likert-scale ratings and Kruskal-Wallis H test results indicated that participants had same level of control and trust on AI-assisted system as non-AI systems as shown in . 
Interestingly, although post-editing did not increase participants' sense of ownership over the  generated headlines, most participants (9/10) in \textit{Guidance + Selection + Post-editing} did edit at least one headline during the task, and the mean of headlines edited was 8.5 ($median = 7.5, std = 6.0$).
%
% It is possible that all participants felt similar ``influence'' over the headlines, in that technically they all did have ``influence''; even in the \textit{Selection} condition, participants made the final headline choice. 

To elucidate the process by which participants post-edited headlines, we provide four examples in Table \ref{tab:editing}. The post-editing changes made by participants were typically minor adjustments, falling into three categories:

\begin{enumerate}
    \item "Hedging": Participants tended to avoid sensationalism or "click-bait" language, opting for more conservative phrasing. For instance, "ruining the environment" was edited to "contributing to climate change", and "expulsion" was revised to "penalties".
    \item Relevance Enhancement: Participants often modified the headlines to make them more pertinent to the target audience, for example, changing "completion" to "climate change".
    \item Fine-tuning: Some edits involved minor adjustments to the text, such as replacing "the state's" with "New Mexico".
\end{enumerate}

From these examples, we discern how participants strategically employed nuanced and effective modifications to enhance the output generated by the AI model. Such human editing data hold the potential to further refine the model through reinforcement learning.
%
% A different experimental design (within-subjects) might have better illuminated subtle differences in control afforded by the different AI assistance. 
% \subsubsection{Edits made by participants in \textit{Guidance + Selection + Post-editing} with post-editing capability}

% \subsubsection{Edits made by participants in \textit{Guidance + Selection + Post-editing} with post-editing capability}

% Most participants (9/10) in \textit{Guidance + Selection + Post-editing} edited at least 1 headline in the post-editing phase ($median = 7.5, mean = 8.5, std = 5.97$).


==> sections/results-prev-2.tex <==
\section{Results}

We report on the results of headline quality (RQ1), task effort---efficiency and perceived difficulty (RQ2), and control and trust (RQ3) for the different AI-assisted text generation conditions.

\subsection{GPT-3.5 only produced the best headlines while manual and selection-only methods produced the worst}
\label{sec:quality}

We compared the quality of the generated headlines between six groups: the four AI-assisted conditions, manual, and automatic methods based on human rankings (see Section~\ref{sec:humaneval}) and collected 2390 rankings (1st to 6th)\footnote{10 codes were missed due to annotator error} from 20 annotators (Table~\ref{tab:eval}). 

The six generated headline groups significantly differed in quality rankings (Kruskal-Wallis H tests, $H-value=50.8, p-value<0.01$). 
Further pairwise comparison of the groups (Table \ref{tab:pairwise_compare}) provides insight into the differences: 
Participants in the \textit{Manual} condition wrote the worst headlines, and \textit{GPT only} produced the best headlines (aside from the \textit{Baseline}).
For the AI-assisted conditions, adding human guidance through providing perspectives (keywords)---(\textit{Guidance + Selection} or \textit{Guidance + Selection + Post-editing})---yielded better headlines than \textit{Selection} alone. 
Post-editing did not impact headline quality: there was no significant difference in ranking between the headlines generated in the \textit{Guidance + Selection} and \textit{Guidance + Selection + Post-editing} conditions.
To further compare the groups, we look at the count of ``top'' (ranked 1st) and ``bottom'' (ranked 6th) rankings (Table~\ref{tab:eval}).
We correctly anticipated the original headlines for the news articles (\textit{Baseline}) would be the highest quality, receiving the most ``top'' rankings (87) and fewest ``bottom'' rankings (38). 
\textit{GPT only}, had fewer ``top'' rankings than \textit{Baseline} (70) but a similar number of ``bottom'' rankings (37). 
\textit{Manual} and \textit{Selection} had the fewest ``top'' rankings (56), while \textit{Manual} also had the most bottom rankings (98).

In Appendix A, Table \ref{tab:casestudy} presents the rankings assigned by one annotator to six headlines, each derived from a different condition, for a single article. Accompanying comments elucidate the rationale behind their ratings—in this case, favoring the succinct headline generated by GPT-3.5 and critiquing the mistake that marred the manually written headline.

To summarize, an approximate comparison of quality ranking among the studied conditions is: \textit{Baseline} $\sim$ \textit{GPT only} > \textit{Guidance + Selection} $\sim$ \textit{Guidance + Selection + Post-editing} > \textit{Selection} $\sim$ \textit{Manual only}.

\begin{table*}[]
\centering
\begin{tabular}{llll}
\hline
\textbf{Condition 1 > Condition 2} & \textbf{U-value} & \textbf{p-value} \\ \hline
\textit{Baseline} > \textit{Manual only} & 61766.0 & <0.01\\
\textit{Baseline} > \textit{Selection} & 63550.0 & <0.01\\
\textit{Baseline} > \textit{Guidance + Selection} & 72364.5 & 0.028\\
\textit{Baseline} > \textit{Guidance + Selection + Post-editing} & 72688.5 & 0.048\\
\textit{GPT only} > \textit{Manual only} & 63168.5 & <0.01\\
\textit{GPT only} > \textit{Selection} & 64751.5 & <0.01\\
\textit{Guidance + Selection} > \textit{Manual only} & 89877.5 & <0.01\\
\textit{Guidance + Selection} > \textit{Selection} & 88536.5 & <0.01\\
\textit{Guidance + Selection + Post-editing} > \textit{Manual only} & 89972.5 & <0.01\\
\textit{Guidance + Selection + Post-editing} > \textit{Selection} & 88734.0 & <0.01\\ \hline
\end{tabular}
\caption{Pairwise comparison of headline quality rankings with significant difference (p<0.05, Mann-Whitney U).}
\label{tab:pairwise_compare}
\end{table*}

\label{sec:efficiency}
\subsection{AI-assisted methods without post-editing were fastest compared to more manual methods}
 
We compare headline generation efficiency using \textit{headline creation time}, i.e., the time to generate the news headline, apart from the time to read the news article--\textit{reading time} (Table \ref{tab:time}).

\begin{figure}
    \centering \includegraphics[width=0.5\textwidth]{figures/Creating.png}
    \caption{News headline creation time across four human conditions (standard deviation as error bars): \textit{Selection} and \textit{Guidance + Selection} are faster than the other two conditions which required more human editing (\textit{Manual} and \textit{Guidance + Selection + Post-editing}).}
\label{fig:creating_time}
\end{figure}

As expected, there was no significant difference in \textit{reading time}.\footnote{While similar average reading time across conditions does not necessarily mean similar engagement and task ability for workers in those conditions, it is a promising indicator.}

The condition did have an impact on \textit{headline creation time}: the \textit{Selection} and \textit{Guidance + Selection} were significantly faster ($H-value=13.0, p-value=0.005$) than the other conditions which involved manual editing (\textit{Manual} and \textit{Guidance + Selection + Post-editing} (see Figure \ref{fig:creating_time}).

\subsection{Condition did not impact task difficulty}
\label{sec:difficulty}

Overall, the participants did not consider the task to be difficult (average instance-level and overall task difficulties are reported in Table \ref{tab:diff}). 

While \textit{Guidance + Selection} had the lowest average instance-level difficulty (M=19.7, SD=24.30) and \textit{Manual} had the highest (M=30.9, SD=17.1), these differences were not significant.

This is surprising as manual methods require more human effort (and time) than writing with assistance. We discuss possible reasons for this finding in the Discussion.

\subsection{Qualitative feedback on AI-assisted headline generation}
\label{sec:comment}
After the task, participants provided open-ended responses as a follow-up to their perceived task difficulty and supplied ``any other comments you want to tell us''.
These responses shed light on perceived benefits of AI assistants, for example to aid brainstorming: 

\begin{quote}
"Overall, I'd say this system could definitely be helpful as long as the keyword list lines up with the main keywords in the article. Additionally, it would always be a helpful brainstorming tool for headlines." (P40, \textit{Guidance + Selection + Post-editing}:)
\end{quote}

Some participants suggested specific considerations for future AI-assisted systems:

\begin{quote}
    \textbf{Coverage of main points in AI-generated headlines:} "Some of the main points were left out of certain headlines, but otherwise, this proves to be a useful tool for journalists. The main points were combined into an easy-to-use database for selection." (P23, \textit{Guidance + Selection})
\end{quote}

\begin{quote}
    \textbf{High efficiency but low creativity and reasoning:} "I could see how this would be beneficial in situations where time is limited, but it does not replace the creativity and reasoning a human has. Some seemed spot on and others seemed chaotic. But with a few tweaks, it was easy to create a headline. Some of the keywords suggested seemed totally unnecessary. The keywords were the weakest part of the system in my opinion." (P39, \textit{Guidance + Selection + Post-editing})
\end{quote}
\begin{quote}
 \textbf{Guidance on AI model and selection of AI outputs as a non-linear process:} "I do wish I could have gone back to choose different perspectives and see alternate variations than just the 3 original headlines. If those first 3 options don't really cover the central theme of the article, it would be nice to go back and choose alternate perspectives to see if it populates a more precise headline. Overall though, this is a great tool to save time and many headaches.
I really enjoyed this experience and would love to participate again in future exercises." (P28, \textit{Guidance + Selection})
\end{quote}

\subsection{Participants felt similar influence over the final outputs and system trust in all conditions}
\label{sec:results_control}

Similar to task difficulty, the condition did not impact perceived control or trust (Table \ref{tab:post-survey}).

Interestingly, although post-editing did not increase participants' sense of ownership over the  generated headlines, most participants (9/10) in \textit{Guidance + Selection + Post-editing} did edit at least one headline during the task, and the mean of headlines edited was 8.5 ($median = 7.5, std = 6.0$).

To elucidate the process by which participants post-edited headlines, we provide four examples in Table \ref{tab:editing}. The post-editing changes made by participants were typically minor adjustments, falling into three categories:

\begin{enumerate}
    \item "Hedging": Participants tended to avoid sensationalism or "click-bait" language, opting for more conservative phrasing. For instance, "ruining the environment" was edited to "contributing to climate change", and "expulsion" was revised to "penalties".
    \item Relevance Enhancement: Participants often modified the headlines to make them more pertinent to the target audience, for example, changing "completion" to "climate change".
    \item Fine-tuning: Some edits involved minor adjustments to the text, such as replacing "the state's" with "New Mexico".
\end{enumerate}

From these examples, we discern how participants strategically employed nuanced and effective modifications to enhance the output generated by the AI model. Such human editing data hold the potential to further refine the model through reinforcement learning.
